Collaborative Diffusion Model for Recommender System

Diffusion-based recommender systems (DR) have gained increasing attention for their advanced generative and denoising capabilities. However, existing DR face two central limitations: (i) a trade-off between enhancing generative capacity via noise injection and retaining the loss of personalized information. (ii) the underutilization of rich item-side information. To address these challenges, we present a Collaborative Diffusion model for Recommender System (CDiff4Rec). Specifically, CDiff4Rec generates pseudo-users from item features and leverages collaborative signals from both real and pseudo personalized neighbors identified through behavioral similarity, thereby effectively reconstructing nuanced user preferences. Experimental results on three public datasets show that CDiff4Rec outperforms competitors by effectively mitigating the loss of personalized information through the integration of item content and collaborative signals.

==> Section/Preliminary.tex <==
\subsection{Diffusion Model}
The diffusion model is a probabilistic generative framework that reduces Gaussian noise iteratively. First, given an input data sample $x_0 \sim q(x_0)$, diffusion model gradually addes noise via forward process using a Gaussian distribution: 
\begin{align}
    q\left(x_t \mid x_{t-1}\right)=\mathcal{N}\left(x_t ; \sqrt{1-\beta_t} x_{t-1}, \beta_t I\right)
\end{align}
where $\beta_t$ represents the hyperparameter indicating the level of Gaussian noise at each timestep $t$. Using the reparameterization trick and the additivity between independent Gaussian distributions, we can directly define the Gaussian distribution that transitions from the initial state $x_0$ to a sample $x_t$ at an arbitrary time step $t$ in a closed form.
\begin{align}
    q\left(x_t \mid x_0\right)=\mathcal{N}\left(x_t ; \sqrt{\bar{\alpha}_t} x_0,\left(1-\bar{\alpha}_t\right) I\right)
    \label{forward}
\end{align}
where $\alpha_t = 1-\beta_t$ and $\bar{\alpha}_t = \prod_{t'=1}^{T} \alpha_{t'}$. 




Second, after finishing the forward process, the diffusion model removes the noise in reverse process using parameterized learned Gaussian distribution:
\begin{align}
    p_\theta(x_{t-1}|x_t) =
\mathcal{N}(\boldsymbol{\mu}_\theta(\mathbf{x_t, t}), \Sigma_\theta(\mathbf{x_t, t}))
\end{align}
At this point, $p_\theta(x_{t-1}|x_t)$ approximates the tractable forward process posteriors:

\begin{align}
& q\left(x_{t-1} \mid x_t, x_0\right) \propto \mathcal{N}\left(x_{t-1} ; \tilde{\boldsymbol{\mu}}\left(x_t, x_0, t\right), \sigma^2(t) I\right), \text { where } \\ & \left\{\begin{array}{l}\tilde{\boldsymbol{\mu}}\left(\boldsymbol{x}_t, x_0, t\right)=\frac{\sqrt{\alpha_t}\left(1-\bar{\alpha}_{t-1}\right)}{1-\bar{\alpha}_t} x_t+\frac{\sqrt{\bar{\alpha}_{t-1}}\left(1-\alpha_t\right)}{1-\bar{\alpha}_t} x_0, \\ \sigma^2(t)=\frac{\left(1-\alpha_t\right)\left(1-\bar{\alpha}_{t-1}\right)}{1-\bar{\alpha}_t}\end{array}\right.
\end{align}
Note that $\Sigma_\theta(\mathbf{x_t, t})$ is set as $\sigma^2(t)I$  for stable learning. The ultimate goal of the diffusion model is to learn the probability distribution of data $p_\theta(x_0) := \int p_\theta(x_{0:T})dx_{1:T}$, where \( p_\theta(x_{0:T}) := p(x_T) \prod^T_{t=1}p_\theta(x_{t-1}|x_t) \) represents the reverse process, denoising through a Markov chain with learned Gaussian transitions \cite{ho2020denoising}. Following this goal, diffusion models are trained by maximizing the variational bound, also known as the Evidence Lower Bound (ELBO), of the likelihood of the input data sample \(x_0\):

\begin{align}
 \log p\left(x_0\right)& = \log \int p\left(x_{0: T}\right) \mathrm{d} \boldsymbol{x}_{1: T} \nonumber \\ 
& =\log \mathbb{E}_{q\left(x_{1: T} \mid x_0\right)}\left[\frac{p\left(x_{0: T}\right)}{q\left(x_{1: T} \mid x_0\right)}\right] \nonumber \\
& \geq \underbrace{\mathbb{E}_{\boldsymbol{q}\left(\boldsymbol{x}_1 \mid \boldsymbol{x}_0\right)}\left[\log \boldsymbol{p}_{\boldsymbol{\theta}}\left(\boldsymbol{x}_0 \mid \boldsymbol{x}_1\right)\right]}_{\text {(reconstruction term) }}-\underbrace{D_{\mathrm{KL}}\left(\boldsymbol{q}\left(\boldsymbol{x}_T \mid \boldsymbol{x}_0\right) \| p\left(\boldsymbol{x}_T\right)\right)}_{\text {(prior matching term) }} \nonumber\\
& -\sum_{t=2}^T \underbrace{\mathbb{E}_{q\left(x_t \mid x_0\right)}\left[D_{\mathrm{KL}}\left(q\left(x_{t-1} \mid x_t, x_0\right) \| p_\theta\left(x_{t-1} \mid x_t\right)\right)\right]}_{\text {(denoising matching term) }} 
&
\end{align}

To train the parameter $\theta$, we only need to consider the reconstruction term and the denoising matching term. Among them, the denoising matching term can ultimately be characterized as minimizing the difference between the means of two distributions, and it can be formulated as follows:

\begin{align}
     &\mathbb{E}_{q\left(x_t \mid x_0\right)}\left[D_{\mathrm{KL}}\left(q\left(x_{t-1} \mid x_t, x_0\right) \| p_\theta\left(x_{t-1} \mid x_t\right)\right)\right] \nonumber\\ 
     = &\mathbb{E}_{q\left(x_t \mid x_0\right)}\left[\frac{1}{2 \sigma^2(t)}\left[\left\|\mu_\theta\left(x_t, t\right)-\tilde{\mu}\left(x_t, x_0, t\right)\right\|_2^2\right]\right]
     \label{eq7}
\end{align}
With the right reparameterization trick, the simplified diffusion model's final loss function is formulated as in Eq.~\eqref{eq7}:


\begin{align}
    \mathcal{L}_{simple} = \mathbb{E}_{t, \mathbf{x}_0, \boldsymbol{\epsilon}}\left[\left\|\boldsymbol{\epsilon}-\boldsymbol{\epsilon}_\theta\left(\sqrt{\bar{\alpha}_t} \mathbf{x}_0+\sqrt{1-\bar{\alpha}_t} \boldsymbol{\epsilon}, t\right)\right\|^2\right]
\end{align}
Note that the model is trained by predicting randomly sampled noises used at time step $t$. The details regarding the reconstruction term are omitted due to space constraints. After training the diffusion model, for data sampling, the model iteratively removes noise starting from Gaussian noise $\mathbf{x}_T \sim \mathcal{N}(0, I) \text{ to }\mathbf{x}_0$:

\begin{align}
& \mathbf{x}_{t-1} = \frac{1}{\sqrt{\alpha_t}}\left(\mathbf{x}_t - \frac{1 - \alpha_t}{\sqrt{1 - \bar{\alpha}_t}} \boldsymbol{\epsilon}_\theta\left(\mathbf{x}_t, t\right)\right) + \sigma_t \mathbf{z}, \quad \text{where} \\
& t = T, \ldots, 1 \text{ and } \mathbf{z} \sim \mathcal{N}(\mathbf{0}, \mathbf{I}) \quad \text{if } t > 1, \quad \text{else } \mathbf{z} = \mathbf{0} \nonumber
& 
\end{align}

\subsection{Diffusion Recommender Model}

Recently, there have been several attempts to apply diffusion to recommender systems, including sequential recommendation \cite{liu2023diffusion, yang2023generate}. However, this paper exclusively focuses on collaborative filtering, similar to DiffRec \cite{wang2023diffusion}. Unlike the original diffusion model, which predicts Gaussian noise $\epsilon$, DiffRec aims to predict observed input data $x_0$. The denoising matching term $\mathcal{L}$ is as follows:


\begin{align}
    \mathcal{L} = &\,\mathbb{E}_{q\left(x_t \mid x_0\right)}\left[\frac{1}{2 \sigma^2(t)}\left[\left\|\mu_\theta\left(x_t, t\right)-\tilde{\mu}\left(x_t, x_0, t\right)\right\|_2^2\right]\right] \nonumber\\
    =&\,\mathbb{E}_{\boldsymbol{q}\left(\boldsymbol{x}_t \mid \boldsymbol{x}_0\right)}\left[\frac{1}{2}\left(\frac{\bar{\alpha}_{t-1}}{1-\bar{\alpha}_{t-1}}-\frac{\bar{\alpha}_t}{1-\bar{\alpha}_t}\right)\left\|\hat{\boldsymbol{x}}_\theta\left(\boldsymbol{x}_t, t\right)-\boldsymbol{x}_0\right\|_2^2\right]
    \label{diffrec_loss}
\end{align}

Note that $\hat{\boldsymbol{x}}_\theta\left(\boldsymbol{x}_t, t\right)$ predict observed user-item interactions $x_0$. For sampling, Eq.~\eqref{forward} is used with small steps $T' < T$ to make $x_{T'}$, and the reverse process is performed using $\hat{x}_{t-1} = \mu_\theta\left(\hat{x}_t, t\right)$ for $t = T, \ldots, 1$, where $\hat{x}_{T}=x_{T'}$.





$$
q\left(\mathbf{x}_{t-1} \mid \mathbf{x}_t, \mathbf{x}_0\right)=\mathcal{N}(\mathbf{x}_{t-1} ; \tilde{\boldsymbol{\mu}}\left(\mathbf{x}_t, \mathbf{x}_0, \mathbf{t}\right), \sigma^2(t) \mathbf{I})
$$
where $\quad \tilde{\boldsymbol{\mu}}\left(\mathbf{x}_t, \mathbf{x}_0,\mathbf{t}\right):=\frac{\sqrt{\bar{\alpha}_{t-1}} (1-\alpha_t}{1-\bar{\alpha}_t} \mathbf{x}_0+\frac{\sqrt{\alpha_t}\left(1-\bar{\alpha}_{t-1}\right)}{1-\bar{\alpha}_t} \mathbf{x}_t \quad$ and $\quad \sigma^2(t):=\frac{(1-\alpha_t)(1-\bar{\alpha}_{t-1})}{1-\bar{\alpha}_t}$

At this point, $p_\theta(x_{t-1}|x_t)$ approximate the tractable forward process posteriors, $q_(x_{t-1}|x_t,x_0)$ = N(x_(t-1);

The diffusion model is a probabilistic generative model that gradually removes Gaussian noise, learning the probability distribution, \( p_\theta(x_0) := \int p_\theta(x_{0:T}) \), given an input data sample \( x_0 \sim q(x_0) \). Note that p_\theta(x_{0:T}) \) := p(x_t) \pi^T_{t=1}p_\theta(x_(t-1)|x_t) is the reverse process (denoising) consistof markov chain with learned guassian transistions. 



Diffusion model is probabilisitc generative model by graduallly removing the gaussian noise, which learns the problabiity distribution, p_\theta(x_0) := \int p_\theta(x_{0:T}, Given an input data sample x_0 ∼ q(x_0)

briefly review diffusion model





==> Section/ProblemFormulation.tex <==
We focus on collaborative filtering with implicit feedback \cite{hu2008collaborative}. Let $\mathcal{R} \in \{0, 1\}^{|\mathcal{U}| \times |\mathcal{I}|}$ be a binary rating matrix, where $\mathcal{U}$ and $\mathcal{I}$ denote a set of users and items, respectively. The $u$-th row of $\mathcal{R}$, denoted as $\mathbf{r}_u \in \{0, 1\}^{|\mathcal{I}|}$, represents the interaction history of user $u$. 
Let $\mathcal{M} \in [0, 1]^{|\mathcal{F}| \times |\mathcal{I}|}$ be a feature matrix for item-side information, where $\mathcal{F}$ denotes the set of item features.
We construct $\mathcal{M}$ using item review words by computing a normalized bag-of-words histogram vector for each item (i.e., $0 \leq m_{ij} \leq 1, \forall i, j$). 
For instance, if a word $f$ appears in four items with counts $[2,0,3,0]$, normalizing by the total sum yields $\mathbf{m}_f = [0.4, 0.0, 0.6, 0.0]$.





Our objective is to develop a novel diffusion recommender model that effectively harnesses user-item interactions and item-side information to bridge the gap between diffusion models and recommender systems. 
% Our proposed model leverages the preferences of real users and pseudo-users established from item content features through a global attention mechanism to create fine-grained preferences for each user.
Our approach effectively mitigates the loss of personalized information stemming from noise accumulation during the forward process and seamlessly integrates rich item-side information into the user-oriented recommendation process.


% too much detailed?
% Let $\mathcal{R} \in \{0, 1\}^{|\mathcal{U}| \times |\mathcal{I}|}$ be a binary rating matrix, where $\mathcal{U}$ and $\mathcal{I}$ denote a set of users and items, respectively \cite{hu2008collaborative}. The $u$-th row of $\mathcal{R}$, denoted as $\mathbf{r}_u \in \{0, 1\}^{|\mathcal{I}|}$, represents the interaction history of user $u$ with items in $\mathcal{I}$. Let $\mathcal{F} \in [0, 1]^{|\mathcal{K}| \times |\mathcal{I}|}$ be a feature matrix for item-side information, where $\mathcal{K}$ denotes the set of item features\footnote{For convenience, we normalize item features such that $0 \leq f_{ij} \leq 1, \forall i, j$.}. Here, we define $\mathbf{f}_{u'} \in [0, 1]^{|\mathcal{I}|}$ as the interaction history of pseudo-user $u' \in \mathcal{K}$, since users' interaction histories can be viewed as co-visits of the items, same as $\mathbf{r}_u$.

% Our objective is to develop a new diffusion recommender model that fully utilizes generative abilities learned from the backward cascaded rating reconstruction. We incorporate global attention mechanisms for both real users and pseudo-users established from item content features. This rich semantic context helps address the loss of personalized information in user interactions caused by the continuous accumulation of noise throughout the forward process.


% previous
% In this paper, we focus on remmendation with implicit feedback \cite{hu2008collaborative}. Consider a system with $U$ users and $I$ items. The user-item interactions are denoted as a binary rating matrix $\mathbf{R} \in \{0, 1\}^{U \times I}$, where 
% the $u$-th row $\mathbf{r}_u \in \{0, 1\}^{I}$ denotes the interaction of user $u$ with the $I$ items. In addition, we denote item-side information as a feature matrix $\mathbf{F} \in \{0, 1\}^{K_{F} \times I}$, where the $i$-th column, i.e., $\mathbf{f}_{:,i}$, denotes the content feature of the $i$-th item. For convenience, we normalize the item features such that $0 < f_{ij} < 1, \forall i, j$. Our objective is to develop a new diffusion model-based recommender system, fully utilizing the generative and denoising ability of the diffusive process while introducing global attention to real users and item features to address the drawback of forgetting personalized information and sparsity issues to further enhance the performance.


% Not necessary for the problem formulation part.

% and feature-item matrix $S \in [0, 1]^{\mathcal{|F|} \times \mathcal{|I|}}$, respectively.  

% collaborative and item-side information , we can make user-item


% We define the pseudo user $f$'s item interaction vector as $S_f = \{s_{f1}, ..., s_{f\mathcal{I}}\}$.

% Let \( D: \mathcal{U} \times \mathcal{I} \rightarrow \mathbb{R}^{\mathcal{|U|} \times \mathcal{|I|}} \) represent the diffusion recommender. The 
% user \( u \) interest probability distribution is denoted as \( X_u \in \mathbb{R}^{\mathcal{|I|}} \), which is predicted by \( D(R_u) \). 
% Let $U^{real}_{u} = \{u' | \text{ top-k}(sim(R_u, R_{u'}))\}$ and $U^{pseudo}_{u} = \{f' | \text{ top-k}(sim(R_u, S_{f'}))\}$ be real and pseudo users for $u$, respectively. We define the pseudo users and real users as those who have the top-k most similar interests with user $u$ (a total of 2k users). 

% interests within the item space (i.e., $\hat{X_u}$) tailored for personalized recommendations to user $u$. This involves aggregating preference information from both real users $U^{real}_{u}$ and pseudo users $U^{pseudo}_{u}$, then combining them with the individual preference of user $u$

==> Section/RelatedWork.tex <==
\subsection{Generative Recommender System}

briefly review Multi-VAE-based, GAN-based and existing diffusion mdoel-based recommender system

\subsection{Generative Recommender With Item Side information}
There are several studies incorporating item-side information into generative recommenders \cite{li2017collaborative, carraro2022conditioned}. This approach aims to overcome limitations of traditional deterministic collaborative filtering (CF) methods, enabling the effective capture of users’ complex, diverse, and uncertain interests within noisy and sparse user-item interactions. Additionally, by leveraging the context obtained from item-side information, deep latent representations of users and items can be generated, outperforming models that rely solely on user-item interactions.

==> Section/test.tex <==
\begin{equation}
\begin{aligned}
& = \underbrace{\mathbb{E}_{q\left({x}_1 \mid x_0\right)}\left[\log p_{\theta}\left(x_0 \mid x_1\right)\right]}_{\text {(reconstruction term) }}-\underbrace{D_{\mathrm{KL}}\left(q\left(x_T \mid x_0\right) \| p\left(x_T\right)\right)}_{\text {(prior matching term) }}\\
& -\sum_{t=2}^T \underbrace{\mathbb{E}_{q\left(x_t \mid x_0\right)}\left[D_{\mathrm{KL}}\left(q\left(x_{t-1} \mid x_t, x_0\right) \| p_\theta\left(x_{t-1} \mid x_t\right)\right)\right],}_{\text {(denoising matching term) }} 
& 
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
& = \underbrace{\mathbb{E}_{q\left(\mathbf{x}__1 \mid \mathbf{x}_0\right)}\left[\log p{\theta}\left(\mathbf{x}_0 \mid \mathbf{x}_1\right)\right]}{\text {reconstruction term}}-\underbrace{D{\mathrm{KL}}\left(q\left(\mathbf{x}_T \mid \mathbf{x}_0\right) | p\left(\mathbf{x}_T\right)\right)}{\text {prior matching term}}\
& -\sum{t=2}^T \underbrace{\mathbb{E}{q\left(\mathbf{x}_t \mid \mathbf{x}_0\right)}\left[D{\mathrm{KL}}\left(q\left(\mathbf{x}_{t-1} \mid \mathbf{x}_t, \mathbf{x}_0\right) | p\theta\left(\mathbf{x}_{t-1} \mid \mathbf{x}_t\right)\right)\right]}{\text {denoising matching term}},
&
\end{aligned}
\end{equation}

==> Source/Section/Abstract.tex <==
Diffusion-based recommender systems (DR) have gained increasing attention for their advanced generative and denoising capabilities. However, existing DR face two central limitations: \textbf{\textit{(i)}} a trade-off between enhancing generative capacity via noise
injection and retaining the loss of personalized information.
\textbf{\textit{(ii)}} the underutilization of rich item-side information.
To address these challenges, we present a \textbf{\underline{C}}ollaborative \textbf{\underline{Diff}}usion model for \textbf{\underline{Rec}}ommender System (\textbf{\proposed}). 
Specifically, \proposed generates \textit{pseudo-users} from item features and leverages collaborative signals from both real and pseudo personalized neighbors identified through behavioral similarity, thereby effectively reconstructing nuanced user preferences.
Experimental results on three public datasets show that \proposed outperforms competitors by effectively mitigating the loss of personalized information through the integration of item content and collaborative signals. 
% Experimental results on three public datasets demonstrate the effectiveness of CDiff4Rec in compensating for the loss of personalized information by leveraging item content and collaborative signals.

%Our code is available at \href{https://anonymous.4open.science/r/CDiff4Rec-477B}{\color{magenta}{https://anonymous.4open.science\allowbreak/r/CDiff4Rec-477B}}.

% Diffusion model (DM)-based recommender systems (RS) have gained increasing attention for their advanced generative and denoising capabilities. However, integrating DMs with RS faces various challenges such as the loss of personalized information during the forward noise-adding process and difficulty in incorporating rich item-side information into user-oriented DM-based RS. To address these challenges, we propose a \textbf{\underline{C}}ollaborative \textbf{\underline{Diff}}usion model for \textbf{\underline{Rec}}ommender System (\textbf{\proposed}). \proposed achieves cascade reconstruction of 
% personalized user preference by leveraging the preference information of all users and \textit{pseudo-users} established from item content features. Initially, we create a large set of pseudo-users from item feature co-occurrence, inspired by the fact that users' interaction 


% histories can be viewed as co-visits of items. This facilitates the efficient integration of item-side information into user-oriented DM-based RS. Moreover, we construct two personalized user sets comprising the top-$K$ real and pseudo users with the most similar interests to each user, respectively, to enhance personalization. Furthermore, we introduce the effective personalized and global attention mechanisms in the backward cascaded rating reconstruction, aiming to incorporate collaborative signals from both real and pseudo users into DM-based RS. Experimental results on three public datasets demonstrate the superiority of \proposed in enhancing recommendation performance. Our code is available at \href{https://anonymous.4open.science/r/\proposed-495C}{\color{magenta}{https://anonymous.4open.science/r/\proposed-495C}}.







% before
% Recently, there has been growing interest in developing recommender systems (RS) based on diffusion models (DMs), where the superior generative and denoising ability of diffusive processes can be fully utilized to enhance the recommendation performance. However, combining DMs with RS faces various challenges, such as loss of personalized information during the forward noise-adding process, and the difficulty in incorporating rich item side information into user-oriented diffusion, etc. In this paper, we propose a novel collaborative diffusion recommender system, i.e., \proposed, aiming to address the above challenges simultaneously. In a nutshell, \proposed design a new recommendation-oriented diffusive process to close the above gaps bwteen DM and RS, where the cascade reconstruction of personalized information in the backward process is achieved by globally attending to all users and \textit{pseudo-users} established from item content features. Specifically, we first establish a large set of pseudo users from the co-occurrence of item features, inspired by the fact that users' interaction histories can be viewed as a co-visit of the items. Through this strategy, item side information can be novelly incorporated into the user-oriented diffusion process to support backforward diffusion. In addition, a novel global attention mechanism over all the real and \textit{pseudo} users is proposed in the backward cascaded rating reconstruction process, where rich global side-information can be effectively incorporated into DMs to preserve and cascadedly reconstruct the personalized information. Experimental results on three public datasets demonstrate the effectiveness of \proposed.



% 최근 Diffusion model을 collaborative filterting에 활용한 모델이 좋은 성능을 보여주고 있다. 그러나 해당 모델은 Diffusion 과정에서 personalized information의 loss를 겪어서 개인화된 추천을 하는데 어려움을 야기한다. 이러한 문제를 해결하기 위해서 우리는 item side information을 활용하여 pseudo user를 생성하였고, 기존에 존재하는 real user와 생성된 pseudo user가 갖는preference information을 활용하여 Diffusion Recommender model의 성능을 더욱 향상시킬 수 있었다. Experiments on three public datasets demonstrate the effectiveness of the proposed method.

==> Source/Section/Conclusion.tex <==
% We propose \proposed, a novel diffusion recommender model that effectively leverages user-item interactions and item-side information to bridge the gap between a diffusion model and recommender system. \proposed utilizes preference information from both real and pseudo-users established from item content features via the global attention mechanism to create a fine-grained interest probability distribution for each user. This approach effectively mitigates the loss of personalized information resulting from noise accumulation during the forward process and seamlessly integrates rich item-side information into the recommendation process. Experimental results on three public datasets demonstrate the effectiveness of \proposed. In the future, we will explore various attention mechanisms to maximize the utilization of rich item-side information in the diffusion recommender model efficiently and effectively.
% We propose \proposed, which integrates preference information from personalized real and pseudo users for each user, established from item content features, into diffusion recommender (DR). Through the global attention mechanism, \proposed creates fine-grained user preference and demonstrates its superiority through extensive experiments on three public datasets. In conclusion, \proposed effectively addresses the loss of personalized information and seamlessly integrates rich item-side information into DR. In future work, we plan to explore multi-modal DR using various types of item features, such as text and images.

% We propose \proposed to effectively address the loss of personalized information and seamlessly integrate rich item-side information into diffusion recommender (DR). \proposed leverages preference information from personalized real and pseudo users through the personalized and global attention mechanism. Experimental results on three public datasets show its superiority. In future work, we will explore multi-modal DR incorporating various item features including text, images, and more.

% In this paper, we propose \proposed, a novel recommender system that seamlessly integrates user-item interactions and item-side content for recommendation via user-oriented diffusion.
% By efficiently converting item content into a large set of pseudo-users and incorporating collaborative signals from both real and pseudo neighbors, 
% \proposed effectively enhances DR by addressing the loss of personalized information.
% Experimental results on three public datasets demonstrate the superiority of \proposed. 
% We believe \proposed lays a strong foundation for leveraging diverse item features in next-generation diffusion-based recommender systems.

%In future work, we will explore multi-modal DR incorporating various item features including text, images, and more.

In this paper, we propose \proposed, a novel diffusion-based recommender system that integrates item content and collaborative signals to mitigate the loss of personalized information. 
By converting item review words into pseudo-users and incorporating the preference information from both real and pseudo personalized neighbors, \proposed effectively reconstructs nuanced user preferences through complementary knowledge.
Experimental results on three public datasets show its superiority, 
while additional analyses suggest that  \proposed achieves a good balance between accuracy and efficiency.
We expect that \proposed will inspire further research on leveraging diverse item-side information to advance existing user-oriented DR.

%We believe CDiff4Rec will inspire future research on leveraging diverse item features and collaborative signals to advance user-oriented DR.
% \vspace{-0.4cm}

==> Source/Section/Experiment.tex <==
\subsection{Experimental Settings}
% \vspace{-0.1cm}
\subsubsection{\textbf{Datasets.}}
We use three public real-world datasets: Yelp\footnote{\url{https://www.yelp.com/dataset}}, Amazon-Game\footnote{\url{https://cseweb.ucsd.edu/~jmcauley/datasets/amazon_v2}}, and Citeulike-t\footnote{\url{https://github.com/js05212/citeulike-t}}. For implicit feedback, we binarize the rating scores of four and five. We then randomly divide the interactions of each user into train/validation/test sets with an 80\% /10\%/10\% split. Table~\ref{Dataset} summarizes the detailed dataset statistics.
%We construct the item feature matrix (i.e., $\mathcal{F}$) by computing tf-idf values from item review data, following \cite{li2017collaborative}.
\vspace{-0.1cm}
\subsubsection{\textbf{Baselines.}}
We compare \proposed with various baselines: traditional CF methods (e.g., BPRMF~\cite{rendle2009bpr} and LightGCN~\cite{he2020lightgcn}), generative model-based CF methods (e.g., MultiVAE~\cite{liang2018variational} and DiffRec~\cite{wang2023diffusion}), a generative method using neighborhood information (e.g., Ease \cite{steck2019embarrassingly}), and a generative method that incorporates item content features (e.g., ConVAE~\cite{carraro2022conditioned}). 
For ablation analysis, we evaluate three versions of \proposed by integrating \textbf{\textit{(i)}} only real neighbors, \textbf{\textit{(ii)}} only pseudo neighbors, \textbf{\textit{(iii)}} and both, as shown in Table~\ref{tab:main_table}.




% The number of the most similar interests with each individual user as top-$K$ real and pseudo-users, respectively, is searched within $\{10, 20, 50\}$.
%The number of pseudo-users (i.e., $|\mathcal{F}|$) is selected from $\{1000, 5000, 10000, 20000\}$.

\vspace{-0.1cm}
\subsubsection{\textbf{Implementation Details.}}
We conduct a grid search on the validation set utilizing PyTorch with CUDA from RTX A6000 and AMD EPYC 7313 CPU.
Our backbone is an MLP with a hidden size of 1,000.
$\alpha, \beta, \text{ and } \gamma$ are explored in the ranges $\{0.1, 0.3, 0.5, 0.7, 0.9\}$. 
The number of top-$K$ neighbors is searched within $\{10, 20, 50\}$. 
The learning rate and weight decay are searched within $[5\mathrm{e}{-5}, 5\mathrm{e}{-4}]$ and $[0.0, 1\mathrm{e}{-4}]$, respectively.
For evaluation, we use Recall@20 (R@20) and NDCG@20 (N@20).
Note that we report results using attention scores based on behavior similarity, which outperforms other approaches (Eq.~\eqref{eq:att}).
The specific parameters of DR are searched 
following the settings in ~\cite{wang2023diffusion}.
All remaining hyperparameters of \proposed are set to default values.
The baseline-specific hyperparameters adhere to the search ranges of original papers.

% The remaining hyperparameters of CDiff4Rec are set to their default values. For baseline-specific hyperparameters, we follow the search ranges provided in the original papers.
% \footnote{We can selectively use real users when $\gamma = 0$, or pseudo-users when $\beta = 0$.}.

\input{Source/Table/small_main_table}

\subsection{\textbf{Performance Comparison}}
Table \ref{tab:main_table} shows that \proposed outperforms all baselines across three datasets.
The results are analyzed from three perspectives: 
\textbf{\textit{(i)}} Generative methods generally surpass traditional ones (i.e., BPRMF and LightGCN), except on Citeulike-t, by effectively capturing the complex and diverse interests of users.
\textbf{\textit{(ii)}} ConVAE, which integrates item features into MultiVAE, outperforms MultiVAE, emphasizing the importance of leveraging item-side information.
\textbf{\textit{(iii)}}  Ease, which incorporates neighborhood information into the generative model,  achieves the best performance among competitors, except on AM-game, highlighting the value of neighborhood-based signals.

Building upon the three aforementioned strengths, \proposed outperforms competitors by effectively mitigating personalized information loss through the integration of item content and collaborative signals from personalized neighbors. 
Notably, CDiff4Rec exhibits a significant performance improvement over DiffRec when employing real neighbors, pseudo neighbors, or both.
This indicates that CDiff4Rec provides DR with complementary knowledge, thereby effectively reconstructing nuanced user preferences.



%established from item content features via the personalized and global attention mechanisms.
% It facilitates the utilization of collaborative signals from these neighbors, enabling a more fine-grained representation of user preferences.
% Therefore, \proposed enhance the effectiveness of DR by addressing the loss of personalized information, as evidenced by a significant performance gap against DiffRec~\cite{wang2023diffusion} when integrating real users, pseudo-users, or both together.

\input{Source/Table/acc_effi}
\input{Source/Table/ablation_topk}

\subsection{\textbf{Study of \proposed}}
\subsubsection{\textbf{Accuracy and efficiency analysis.}}
We compare the accuracy and efficiency of DiffRec and \proposed using Recall (R), NDCG (N) at 10, 50, 100.
Here, wall time is the total elapsed time for model execution, including both training and inference. 
Table~\ref{tab:acc_eff} shows that \proposed consistently outperforms DiffRec across the three datasets with negligible additional overhead.
An analysis of each dataset is as follows:
On Yelp, \proposed improves R@10 by 12.3\% and N@10 by 12.1\%, while wall time increases by just 10.5\%, showing a favorable trade-off between accuracy and computational cost.
On Amazon-Game (AM-Game), \proposed consistently achieves higher scores across all metrics, despite having a wall time similar to that of DiffRec.
On Citeulike-t, \proposed maintains comparable accuracy yet converges faster, indicating improved efficiency.
Overall, these results suggest that \proposed achieves a better balance between accuracy and efficiency than DiffRec.

\subsubsection{\textbf{Hyperparameter study.}}
We investigate the impact of varying  the number of \textbf{\textit{(i)}} top-$K$ neighbors and \textbf{\textit{(ii)}} pseudo-users (i.e., review words).
Here, pseudo-users are selected based on the highest average TF-IDF scores across multiple items, computed as follows:
\vspace{-0.1cm}
\begin{equation}
    \begin{aligned}
        \text{avg}_\text{TF-IDF}(f) = \frac{1}{|\mathcal{I}|}\Sigma^\mathcal{|I|}_{i=1}\text{TF-IDF}(f,i).
    \end{aligned}
\end{equation}
Table \ref{topk} presents that \proposed overall shows superior performance with top-$20$ neighbors and 1,000 pseudo-users across the three datasets.
This result suggests that CDiff4Rec effectively balances accuracy and efficiency, achieving strong performance even with a relatively small number of top-$K$ neighbors and pseudo-users.


% consistently achieves superior performance with a strategic selection of top-$K$ neighbors and a reasonable number of pseudo-users. 
% Specifically, when the quantity of pseudo-users is set to 1,000 and $K$ is set to 20, \proposed shows superior performance. 
% This highlights that \proposed achieves efficient and effective performance even with a small number of item features as pseudo-users and appropriately selected top-$K$ neighbors.
% can utilize a small number of item features as pseudo-users and leverage the preference information of appropriate top-$K$ real and pseudo users, validating its efficiency and effectiveness.
% This suggests that \proposed can utilize a small number of item features as pseudo-users and leverage the preference information of appropriate top-$K$ real and pseudo users, validating its efficiency and effectiveness.


==> Source/Section/Introduction.tex <==

Recommender systems have become indispensable tools for 
helping users make informed decisions by delivering personalized recommendations amidst the overwhelming information on the Web~\cite{ricci2010introduction,zhu2024collaborative}. A widely adopted strategy in RS is collaborative filtering (CF), which models user preferences based on user-item interactions through traditional methods (e.g., matrix factorization~\cite{koren2009matrix, he2017neural} and graph neural networks~\cite{wang2019neural, he2020lightgcn}). 
% gnerative
Moreover, deep generative models further enhance CF by effectively capturing user preferences in noisy and sparse interactions through their generative capabilities~\cite{harshvardhan2020comprehensive,wu2016collaborative} (e.g., Generative Adversarial Networks (GANs)~\cite{wang2017irgan, chae2018cfgan} and Variational Autoencoders (VAEs)~\cite{liang2018variational,zhu2022mutually}).
However, these generative models face significant challenges: GANs are prone to unstable training~\cite{xu2020understanding}, while VAEs often suffer from posterior collapse, limiting their ability to model user preferences accurately~\cite{liu2022hybrid}. 

Recently, diffusion models introduce a novel generation paradigm
by progressively adding Gaussian noise to inputs \textit{(forward process)} and reconstructing them via a parameterized Markov chain \textit{(backward process)}.
With their capability to significantly enhance generative quality and stability~\cite{ho2020denoising, luo2022understanding}, 
diffusion-based recommender systems (DR) have been explored for higher-quality recommendations~\cite{yang2024generate, li2023diffurec, du2023sequential, wu2023diff4rec, liu2023diffusion, wang2023diffusion, han2024controlling}. 
For example, DreamRec~\cite{yang2024generate} utilizes guided diffusion to generate oracle items in sequential recommendation (SR). DiffuASR~\cite{liu2023diffusion} mitigates the challenges of data sparsity and long-tail user problems in SR.
DiffRec~\cite{wang2023diffusion} is the first to apply DR to CF by denoising corrupted user-item interactions.

% 문제점을 더 극명하게 쓰자.
However, existing DRs still encounter two major challenges: 
\textbf{\textit{(i)}} a dilemma between maximizing generative capacity via noise injection and the loss of personalized information, and \textbf{\textit{(ii)}} the underutilization of item-side information.
First, DR faces a dilemma: Excessive noise-adding operations transform inputs into pure noise, causing substantial loss of personalized information and complicating the reconstruction of user preferences, whereas insufficient noise limits generative capabilities.
Although reducing noise levels or diffusion steps can partially reconcile this trade-off~\cite{wang2023diffusion}, performance remains highly sensitive to hyperparameters and prone to inconsistency.
Second, the user-oriented nature of DR leaves the integration of rich item-side information (e.g., item reviews) underexplored, limiting their potential to fully leverage complementary knowledge sources for more accurate recommendations.

To address these challenges, we propose a \textbf{\underline{C}}ollaborative \textbf{\underline{Diff}}usion model for \textbf{\underline{Rec}}ommender System (\textbf{\proposed}). 
The goal of \proposed is to mitigate the loss of personalized information by leveraging item-side information and collaborative signals (i.e., latent knowledge derived from behavioral similarity between users).
Specifically, \proposed operates in three main steps: 
First, we generate \textit{pseudo-users} from item features (i.e., review words) by treating each feature (i.e., a word) as a pseudo-user based on its co-occurrence across multiple items (e.g., a word appears in the reviews of different items).
Thus, the interaction history of a pseudo-user is analogous to a user's interaction history spanning multiple items.
Second, for each real user (query user), we identify two types of personalized top-$K$ neighbors—one from real users and another from pseudo-users—based on behavioral similarity.
Finally, during the diffusion process, we incorporate the preference information from both real and pseudo neighbors to 
generate a fine-grained representation of the query user's preferences.
This integration of item content and collaborative signals substantially enhances the cascade reconstruction in DR.
Experimental results on three public datasets show that \proposed outperforms various baselines.
Our additional analyses support the effectiveness of each proposed component.



% aiming to bridge the gap between DM and RS by mitigating the loss of personalized information and incorporating item-side information into user-oriented DM-based RS. \proposed facilitates the cascade reconstruction of personalized user preference during the backward diffusive process by leveraging the preference information from all users and pseudo-users established from item content features. Specifically, we first create a large set of pseudo-users from item feature co-occurrence, inspired by the fact that users' interaction histories can be viewed as co-visits of the items. This enables the efficient integration of item-side information into user-oriented DM-based RS. Moreover, we construct two personalized user sets comprising the top-$K$ real and pseudo users with the most similar interests to each individual user, respectively, to enhance personalization. Furthermore, we introduce the effective personalized and global attention mechanisms over all the real and pseudo-users during the backward cascaded rating reconstruction process. This strategy enables the seamless incorporation of the preference information from both real users and pseudo-users into \proposed as collaborative signals for better personalized recommendations. The performance comparison on three public datasets demonstrates \proposed's superiority over baselines. 


% Additionally, the ablation study validates its efficiency and effectiveness by varying the number of top-$K$ users with the most similar interests to each user and the quantity of pseudo-users.
% Additionally, the ablation study validates the efficiency and effectiveness of CDiff4Rec by varying the number of top-$K$ similar interest users and adjusting the quantity of pseudo-users.



%Experimental results on three public datasets demonstrate the superiority of \proposed in enhancing recommendation performance.




% Recommender systems (RS) have been widely employed across various online platforms to facililate users' decisions in the era of information overload \cite{ricci2010introduction}. One widely-used strategy for RS is collaborative filtering (CF), which aims to model user interests based on their past interactions \cite{he2017neural}. Traditional CF-based methods include matrix factorization (MF) \cite{koren2009matrix} or neural networks \cite{he2020lightgcn}. Recently, generative RSs have attracted more attention from researchers, which can more effectively capture users' complex, diverse, and uncertain interests in noisy and sparse user-item interactions \cite{harshvardhan2020comprehensive}.


% Deep generative models, e.g., variational auto-encoder (VAE) and generative adversarial network (GAN), have been widely adopted for generative CF-based RSs \cite{harshvardhan2020comprehensive}. One exemplar method is the MultiVAE \cite{liang2018variational}, which uses VAE with multinomial likelihood to generate user's historical interactions. Additionally, IRGAN \cite{wang2017irgan} adapts GAN for RS by generating ratings with an adversarial discriminator. However, these generative models often face challenges such as unstable training (for GAN-based methods) and may fail to adequately model user preferences within their hidden representations when posterior or mode collapse occurs (for VAE-based methods). 

% Needs more methods.
% Recently, diffusion models (DMs) introduce a novel diffusive generation paradigm, where noise is cascadely added on the input (forward process) and is iterative reconstructed back (reverse process), such that the generation quality and stability can be substantially improved \cite{ho2020denoising}. Therefore, there have been a few explorations to integrate DMs with RS, fully utilizing  superior generation ability of DM to support recommendations. Specifically, DiffRec \cite{wang2023diffusion} extends conventional DMs to collaborative filtering by corrupts users' interaction histories by adding Gaussian noise and denoises them using a parameterized neural network. However, these methods still face two major challenges as follows: First, since DMs cascadedly add noise on user ratings before reconstruction, auxiliary information in the  user ratings can be lost, which hinders effective reconstruction of user interest for new item recommendations. In addition, since existing diffusion-based RS follows a user-oriented denosing process by cascadely denoise the user ratings, rich item side information cannot be incorporated to further support recommendations. 

% To address this problem, we propose a collaborative diffusion recommender (CDiff4Rec), aiming to close the gap between DM and RS by addressing the loss of personalized information and the incorporation of item side information simultaneously. CDiff4Rec facilitates the cascade reconstruction of personalized information in the backward diffusive process by globally attending to all users and \textit{pseudo-users} established from item content features. Specifically, we first establish a large set of pseudo users from the co-occurrence of item features, inspired by the fact users' interaction history can be viewed as a co-visit of the items. In addition, a novel global attention mechanism over all the real and pseudo users is proposed in the backward cascaded rating reconstruction process. Through this strategy, personalized information and rich item content information can be effectively incorporated into the diffusion model for better recommendations. Experimental results on three public datasets demonstrate the effectiveness of the proposed CDiff4Rec.

% Our contributions can be summarized as follows:

% \begin{itemize}
%     \item We introduce CDiff4Rec to overcome personalized information loss in DiffRec \cite{wang2023diffusion} by creating a fine-grained user interest probability distribution.
%     \item To implement this, we utilize item side information to generate pseudo users and extract preference information from both existing real users and generated pseudo users.
%     \item Experimental results on three public datasets demonstrate the effectiveness of our proposed approach and enhance DiffRec's \cite{wang2023diffusion} personalized recommendations.
% \end{itemize}



% 다양한 플랫폼에서 추천 시스템을 활용하여 사용자에게 맞춤형 추천을 제공하고 이를 통해 플랫폼 수익을 증가시키는 노력들이 최근 두드러지고 있습니다. 추천 시스템의 궁극적인 목표는 사용자의 관심을 정확하게 모델링하여 개인화된 추천을 수행하여 소비자의 만족도를 극대화하는 것에 있습니다. 이를 위해 기존의 MF나 GCN 기반 모델들은 사용자와 아이템의 표현을 적절히 모델링하는 것을 목표로 학습되지만, 추천 시스템에서 사용되는 데이터는 소음과 희소성과 같은 문제를 가지고 있기 때문에 단순히 user-item의 interaction만을 가지고 고정된 representation 형태로 user/item을 표현하는 방식은 사용자의 복잡하고, 다양하고, uncertain한 관심사를 제한적으로 반영한다는 한계점이 있습니다.


% 최근에는 생성 모델을 추천 시스템에 적용하려는 여러 시도들이 두드러지는 성능을 보여주고 있습니다. 이러한 생성 모델들은 user interaction probabilities를 학습하여 Item-space상에 존재하는 모든 item들에 대한 user의 interest의 정도를 효과적으로 모델링할 수 있어서 사용자의 숨겨진 관심사를 추론할 수 있기에, 기존 representation기반의 추천 시스템이 가지는 한계들을 잘 극복할 수 있습니다.

% 구체적으로, VAE를 활용하여 기존의 autoencoder 구조에 multinomial likelihood function parameterized by neural network하여 modeling user-item implicit feedback data하였습니다. 또한 GAN을 이용하여 판별 모델과 생성 모델 간의 경쟁을 통해 주어진 데이터의 확률 분포를 학습하고 이후, 사용자와 아이템의 latent vectors를 추출하여 아이템을 추천하는 방식도 제안되었습니다.

%  그러나 이러한 생성 모델들은 학습이 불안정하고 posterior 또는 mode collapse로 인하여 hidden  representation이 user의 preference를 적절히 반영하지 못한다는 한계를 가지고 있습니다.

% 최근에는 Diffusion 모델이 iterative한 방식으로 소음을 제거하면서 안정적으로 데이터의 확률 분포를 학습하여 기존 생성모델에 앞서는 성과를 보여주고 있으며, 추천 시스템에서도 협업 필터링 및 순차적 추천에 활용되고 있습니다. 

% 그러나 디퓨전 과정에서 noise를 반복적으로 더함으로써 발생하는 personalized information의 손실로 인해 적절한 추천이 이뤄지지 않는다는 문제가 있습니다. 기존논문은 이 문제를 해결하기 위해서 noise의 수준을 낮추거나, 추론 과정에서 디퓨전 단계의 수를 줄이는 수동적인 방식으로 해결되었지만, 근본적으로 이 문제를 해결하지 못했습니다.

% 따라서 우리는 이러한 한계를 극복하고자 item의 side information을 활용하는 강화된 Diffusion model의 방식을 제안하게 되었습니다. 구체적으로는 아이템 특성 행렬을 사용하여 가상의 사용자를 생성하였습니다. 이후,

%  기존의 실제 사용자와 생성된 가상 사용자로부터 나오는 preference information을 추출하여 이를 각 사용자가 갖는 선호도를 고려하여 사용자의 세부적인 사용자-아이템 상호작용 확률분포를 생성할 수 있었습니다.

% 우리의 기여를 요약하면 다음과 같습니다.

% 1.	우리는 DiffRec이 가지는 personalized information loss의 한계를 극복하기 위해 Item side information을 활용하여 가상 사용자를 생성하였고, 기존 사용자와 생성된 가상 사용자로부터 preference information을 적절히 추출하여 각 user의 fine-grained한 user interest probability를 생성해낼 수 있었습니다.
% 2.	3개의 공공 데이터셋에 대한 실험을 통해 우리의 방법의 효과를 입증했습니다.




% 많은 플랫폼에서 추천시스템을 활용하여 유저로 하여금 개인화된 추천을 이루고, 플랫폼의 수익을 증대시켜나가고 있다. 이러한 추천시스템의 근본적인 목적은 유저의 interest를 적절히 모델링하여 개인화된 추천을 수행하는 것에 있다. 이를 위해서 MF, GCN 기반의 기존의 모델들은 유저와 item의 representation을 적절히 모델링하는 것을 목표로 학습이 진행된다. 그러나 이와 같은 표현은 user의 복잡한 interest를 모델링하는 것에 상당한 제약을 둘 수 밖에 없다. 왜냐하면 이와 같은 고정된 형태의 vector로 표현해내는 것은 

% representation은 유저의 diverse / complex / uncertatin한 interest를 제한적인 형태로 반영하고 있기 때문이다.
% 또한 추천시스템에서 사용된 데이터가 가지는 noisy함과 sparsity와 같은 문제를 지니고 있기 때문에, user와 item의 interaction을 is the most relevant one으로 두는 것은 exposure bias에 취약하게 만들어서 종국에는 user의 underlying interest를 catch하는것에 어려움을 초래한다.

% 최근 생성모델을 활용하여 추천시스템에 접목시키려는 여러 시도들이 돋보이고 있다. 
% 이러한 생성모델들은 데이터의 확률분포를 학습하여 user의 숨겨진 interest를 적절히 모델링 하는데 능숙하기 때문에, 추천시스템의 특성을 적절히 고려하고 있다.

% 대표적으로 VAE를 활용하여 기존의 autoencoder구조를 기반으로 latent variable에 a multinomial likelihood function을 모델링하여 좋은 성능을 보여주기도 하였다.  [Mult-VAE]. 

% 또한, GAN을 활용하여 dicriminative model과 generative model의 경쟁을 통해 확률분포를 학습시키고 이후, user와 item의 latent vectors를 extracting하여 item을 추천하는 방식을 보여주기도 하였다 [IRGAN]

% 그러나 이와 같은 VAE, GAN과 같은 생성모델은 학습이 불안정하고, posteior / mode collapse에 빠져서 latent knowledge가 적절히 modeling되지 않을 수 있다는 한계를 가진다.

% 최근 Diffusion model이 생성모델에서 눈부신 활약을 iterative manner로 noise를 제거하면서 안정적으로 데이터의 확률분포를 학습해 나가는 모습을 보여주고 있고, 추천시스템에서도 collabrative filtering, sequential recommendation에 활용되고 있다. 
% 그러나 디퓨전 과정에서 발생하는 personalized information의 loss로 인해 적절한 추천이 이뤄지지 않는 문제가 존재한다. 기존 기존 모델은 noise의 level을 낮추거나, inference과정에서 diffusion의 step의 수를 줄이는 manual한 방식으로 이를 해결하였으나, 이는 근본적으로 해당 문제를 해소시키지 못한다.

% 따라서 우리는 추가적인 정보를 활용해서 이러한 한계를 극복하고자 하였다. 구체적으로 item-feature matrix를 활용하여 pseudo user를 생성하였고, 기존의 real user 그리고 생성된 pseudo user로부터 오는 추가적인 정보를 활용하여 각 user의 preference를 적절히 모델링하여 궁극적으로는 personalized recommendation이 가능하도록 diffrec을 향상시킬 수 있었다. 이를 위해서 우리는 하나의 user와 real user / 하나의 user와 pseudo user간의 관계를 고려하였고, top-k similar interest를 가지는 real users, pseudo users를 활용하여 각 user의 fine-grained한 user-item interaction score를 생성할 수 있었다.

% 우리의 contribution을 요약하면 아래와 같다.
% 1. 우리는 DiffRec이 갖는 personalized information loss의 한계를 극복하기 위해서 추가적인 정보를 적극적으로 활용하여, 기존 user와 생성된 psuedo user로 부터 fine-grained한 정보를 활용할 수 있었다.

% 2. pseudo user의 생성을 위해서 item-side information을 활용하였다.

% 3. 3개의 public dataset에 대한 실험을 통해 우리 method의 우수성을 보여주었다.


% # 추천시스템 자체

% # 기존의 모델 -> 한계
    % 유저와 아이템이 제한된 형태로 표현될 수 밖에 없다.
    % 추천시스템이 가지는 

% # 생성모델의 활용 -> 한계
    % VAE, GAN과 같은 모델들은 학습이 불안정하고, posteior / mode collapse에 빠져서 latent knowledge가 적절히 modeling되지 않을 수 있음

% # 디퓨전 모델의 활용 -> 한계
    % 최근 Diffusion model이 생성모델에서 눈부신 활약을 iterative manner로 noise를 제거하면서 안정적으로 데이터의 확률분포를 학습해 나가는 모습을 보여줌
    % 추천시스템에서도 이러한 Diffusion 모델의 활용
        % 그러나 디퓨전 과정에서 발생하는 personalized information의 loss로 인해 적절한 추천이 이뤄지지 않음. 기존 모델은 noise의 level을 낮추거나, inference과정에서 diffusion의 step의 수를 줄이는 manual한 방식으로 

% # 우리의 제안

% # 우리의 contribution (side information, relation을 활용, 실험으로 이를 보여줌)

% are utilized to infer the user interaction probabilities over non-interacted items. These models use a generative process in which the user preferences are considered latent factors that determine users’ interaction behaviors. Sampling from the learned probability distribution mimics the uncertainty of user behavior.

==> Source/Section/Method.tex <==
In this section, we introduce a \textbf{\underline{C}}ollaborative \textbf{\underline{Diff}}usion model for \textbf{\underline{Rec}}ommender System (\textbf{\proposed}) (see Figure~\ref{fig:main_figure}). 
CDiff4Rec consists of three stages: \textbf{\textit{(i)}} generation of pseudo-users from item review data (\cref{sub:pseudo_user}), \textbf{\textit{(ii)}} identification of two types of personalized top-$K$ neighbors from real and pseudo-users (\cref{sub:ident_topk}), and \textbf{\textit{(iii)}} aggregation of collaborative signals from those neighbors by incorporating their preference information during the diffusion process (\cref{sub:agg_col}).

% \subsection{Forward Process} \label{sec:forward_process}
% % In the forward process of diffusion recommender (DR), a Gaussian noise is continuously added to user-item interactions over timestep. 
% Let $\mathbf{r}_u$ represent the input $\mathbf{x}_0$ of diffusion recommender (DR) at timestep $t = 0$. When $\mathbf{x}_0$ is fed into DR, Gaussian noise is continuously added from $\mathbf{x}_0$ to $\mathbf{x}_t$ step by step over timestep $t$, following a Markov process:
% % the model corrupts the user-item interaction using Gaussian probability distributions step by step over timestep $t$ as a Markov process:
% \vspace{-0.15cm}
% \begin{equation}
% \begin{aligned}
%     q\left(\mathbf{x}_t \mid \mathbf{x}_{t-1}\right)=\mathcal{N}\left(\mathbf{x}_t ; \sqrt{\alpha_t} \mathbf{x}_{t-1}, (1-\alpha_t) \boldsymbol{I}\right),
% \end{aligned}
% \vspace{-0.15cm}
% \end{equation}
% where $\mathbf{x}_t$ is a corrupted interaction during the forward noise-adding process and $\alpha_t$ represents a hyperparameter indicating the level of Gaussian noise at timestep $t$. Utilizing the properties of Gaussian distribution \cite{ho2020denoising, luo2022understanding, wang2023diffusion}, we can directly define a distribution that transits from the initial state $\mathbf{x}_0$ to the corrupted data $\mathbf{x}_t$ at an arbitrary timestep $t$ in a closed form, enabling an efficient forward process:
% \vspace{-0.15cm}
% \begin{equation}
% \begin{aligned}
%     q\left(\mathbf{x}_t \mid \mathbf{x}_0\right)=\mathcal{N}\left(\mathbf{x}_t ; \sqrt{\bar{\alpha}_t} \mathbf{x}_0,\left(1-\bar{\alpha}_t\right) \boldsymbol{I}\right),
%     \label{forward}
% \end{aligned}
% \vspace{-0.15cm}
% \end{equation}
% where $\bar{\alpha}_t = \prod_{t'=1}^{T} \alpha_{t'}$. However, existing DR encounters the challenge of personalized information loss during the forward noise-adding process. Despite the attempts to address this issue by reducing noise levels or decreasing diffusion steps for inference \cite{wang2023diffusion}, these manual techniques not only lack efficiency and effectiveness but also have the potential to compromise the efficacy of DR.

% these ad-hoc techniques are not only ineffective in addressing this issue but also have the potential to compromise the efficacy of DR.
% \[ q(x_t | x_0) = \mathcal{N}(x_t ; \sqrt{\bar{\alpha_{t}}}x_0, (1-\bar{\alpha_{t}})I) \]

% $\mathcal{N}\left(x_{t-1} ; \tilde{\boldsymbol{\mu}}\left(\boldsymbol{x}_t, \boldsymbol{x}_0, t\right), \sigma^2(t) \boldsymbol{I}\right)$
\vspace{-0.2cm}
\subsection{Pseudo-User Generation from Item Reviews}
\label{sub:pseudo_user}
To effectively mitigate the loss of personalized information in user-oriented DR, 
we strategically leverage item features.
Specifically, we generate pseudo-users by treating each feature (i.e., a review word) as an individual user with a unique interaction history.
Let $pu$ denote a pseudo-user corresponding to a specific feature $f$ (i.e., $pu = f \in \mathcal{F}$), and $ru$ denote a real user (i.e., $ru = u \in \mathcal{U}$).
For each pseudo-user, we construct a vector $\mathbf{m}_{pu} \in [0, 1]^{|I|}$ by processing the original feature vector $\mathbf{m}_f \in \mathbb{R}^{|\mathcal{I}|}$ as follows: First, we apply TF-IDF to compute the importance of the feature for each item.
Then, we perform Min-Max normalization to scale values into $[0, 1]$.
%(i.e., $\mathbf{m}_f \text{ } \raisebox{-0.7ex}{\(\xrightarrow{\text{ TF-IDF, Min-Max }}\)} \text{ }\mathbf{m}_{pu}$).

Here, $\mathbf{m}_{pu}$ is the normalized interaction vector of a pseudo-user, which encodes the relevance of feature $f$ across all items. 
This is analogous to a real user’s binary interaction vector $\mathbf{r}_{ru} \in \{0, 1\}^{|\mathcal{I}|}$, which is the co-visit history of a user $u$ across all items.
We emphasize two advantages of leveraging item features as pseudo-users: 
First, $\mathbf{m}_{pu}$ can be seamlessly incorporated into the existing CF framework based on implicit feedback without requiring specialized loss functions for item features.
%
Second, introducing pseudo-users into DR yields mutual benefits:
DR’s advanced denoising capabilities can reduce noise in the normalized pseudo-user vectors, selectively leveraging the most salient item content.
Meanwhile, the rich item-side information from pseudo-users complements user-oriented signals, contributing to a more accurate reconstruction of user preferences.
% incorporating pseudo-users into DR creates synergistic effects: DR can leverage their advanced denoising capabilities to reduce noise in the normalized interaction vectors of pseudo-users and selectively utilize item content.
% Simultaneously, the rich item-side information provides DR with complementary knowledge, thereby enhancing the reconstruction of user preferences.
Thus, using DR with pseudo-users yields synergistic effects, ultimately enhancing recommendation quality.

%Thus, the synergy of incorporating item-side information through pseudo-users into DR yields significant benefits.

% Second, diffusion recommender (DR) facilitates the selective utilization of meaningful context from noise within pseudo-users, thanks to its robustness to noise \cite{wang2023diffusion}. Therefore, the synergy resulting from the integration of pseudo-users with DR can be significant.

% \vspace{-5pt}
\vspace{-0.2cm}
\subsection{Personalized Top-$K$ Neighbors Identification}
\label{sub:ident_topk}
With the newly generated pseudo-users, we identify two personalized user sets for each query user $u \in \mathcal{U}$: one from real users and the other from pseudo-users.
To determine the top-$K$ neighbors based on behavior similarity, we employ a distance function $\phi: \mathbb{R}^{|\mathcal{I}|} \times \mathbb{R}^{|\mathcal{I}|} \rightarrow \mathbb{R}$. 
In this work, we use cosine distance as: 
\vspace{-0.1cm}
\begin{equation}
    \begin{aligned}
        \mathcal{U}^u_{ru} & = \{ru \,|\, \underset{ru \in \mathcal{U}}{\text{argsort }} \phi(\mathbf{r}_u, \mathbf{r}_{ru})[:K] \}, \\
        \mathcal{U}^u_{pu} & = \{pu \,|\, \underset{pu \in \mathcal{F}}{\text{argsort }} \phi(\mathbf{r}_u, \mathbf{m}_{pu})[:K] \},
    \end{aligned}
    \vspace{-0.1cm}
    \label{make_user}
\end{equation}
where $\mathcal{U}^u_{ru}$ and $\mathcal{U}^u_{pu}$ are the top-$K$ neighbors from real and pseudo-users for query user $u$.
Note that $\mathcal{U}^u_{ru}$ and $\mathcal{U}^u_{pu}$ 
are precomputed and cached during preprocessing, allowing for efficient utilization without additional computation in model training and inference.
\vspace{-0.2cm}
\subsection{Collaborative Signals Aggregation Using PI}
\label{sub:agg_col}
Throughout the diffusion process (forward and then backward), DR generates user interactions by
transforming $\mathbf{r}_u$ into $\hat{\mathbf{r}}_u$, which is represented as $\hat{\textbf{x}}_\theta\left(\textbf{x}_t, t\right) = \hat{\mathbf{r}}_u$ (Eq.~\eqref{eq:diffrec_loss}). 
However, $\hat{\mathbf{r}}_u$ is insufficient because excessive noise erodes personalized information, while limited noise reduces the generative capabilities required to capture latent user preferences.
To address this, we aggregate collaborative signals from two sets of top-$K$ neighbors (i.e., $\mathcal{U}^u_{ru}$ and $\mathcal{U}^u_{pu}$) by incorporating their preference information (PI) during the diffusion process.
This approach yields a fine-grained representation of user preferences, denoted as ${\hat{\mathbf{r}}_u}'$, as follows:
\vspace{-0.1cm}
\begin{equation}
\label{eq:fg_obj}
    \begin{aligned}
        {\hat{\mathbf{r}}_u}' & = \alpha \hat{\mathbf{r}}_u + 
        \beta \underbrace{\sum_{ru_i \in \mathcal{U}^u_{ru}} a_{ru_i}\hat{\mathbf{r}}_{ru_i}}_{\text {PI from real neighbors}} +
        \gamma \underbrace{\sum_{pu_j \in \mathcal{U}^u_{pu}} a_{pu_j}\hat{\mathbf{m}}_{pu_j}}_{\text {PI from pseudo neighbors}},
    \end{aligned}\vspace{-0.1cm}
\end{equation}
where $\alpha$, $\beta$, and $\gamma$ (with $\alpha+\beta+\gamma = 1$) are hyperparameters that control the weights of the user's own, real neighbors, and pseudo neighbors. 
$\hat{\mathbf{r}}_{ru_i} \in \mathbb{R}^{|\mathcal{I}|}$ and $\hat{\mathbf{m}}_{pu_j} \in \mathbb{R}^{|\mathcal{I}|}$ denote the predictions for a real neighbor and a pseudo neighbor, 
while $a_{ru_i}$ and $ a_{pu_j}$ represent their corresponding attention scores.
% are the attention scores of real neighbor $ru_i$ and pseudo neighbor $pu_j$, respectively.
%Let $\mathcal{A}^u_{ru} = \{a^u_{ru_1}, \ldots, a^u_{ru_K}\}$ be a set of attention scores for $\mathcal{U}^u_{ru}$. It consists of individual attention scores $a^u_{ru_k}$ for each real user $ru_k \in \mathcal{U}^u_{ru}$, satisfying $0 \leq a^u_{ru_k} \leq 1$ for $k \in [1, K]$, with $\sum_{k=1}^{K} a^u_{ru_k} = 1$. 
Here, we introduce three approaches to compute these  scores for $a_{ru_i}$, and the same process applies to $a_{pu_j}$: \textbf{\textit{(i)}} average pooling, \textbf{\textit{(ii)}} behavior similarity, and \textbf{\textit{(iii)}} parametric modeling.
Each method is detailed below.
\small{
\begin{equation}
\begin{aligned}    
a_{ru_i} = \begin{cases} \frac{1}{K}, & \text {if average pooling, } \\
\frac{\exp(-\phi(\mathbf{r}_u, \mathbf{r}_{ru_i}))}{\sum_{ru_i \in \mathcal{U}^u_{ru}}\exp(-\phi(\mathbf{r}_u, \mathbf{r}_{ru_i}))}, & \text {if behavior similarity, } \\ 

\frac{\exp((\mathbf{W}_q^T \hat{\mathbf{r}}_u)^T (\mathbf{W}_k^T \hat{\mathbf{r}}_{ru_i}))}{\sum_{ru_i \in \mathcal{U}^u_{ru}}\exp((\mathbf{W}_q^T \hat{\mathbf{r}}_u)^T (\mathbf{W}_k^T \hat{\mathbf{r}}_{ru_i}))}, & \text {if parametric modeling, }\end{cases}
\end{aligned}
\label{eq:att}
\end{equation}
}\normalsize
where $\mathbf{W}_q, \mathbf{W}_k \in \mathbb{R}^{|\mathcal{I}| \times d}$ are parametric weights, with $d$ as the dimensionality. 
We elaborate on the advantages of each approach: \textbf{\textit{(i)}} Average pooling offers straightforward implementation due to its simplicity. 
\textbf{\textit{(ii)}} Pre-calculated distances based on behavior similarity from Eq.~\eqref{make_user} enhance reusability and better reflect actual user similarity by leveraging the observed interaction history ($\mathbf{r}_{u}$).
\textbf{\textit{(iii)}} Parametric modeling effectively learns user relationships by using cascaded reconstructed interactions ($\hat{\mathbf{r}}_{u}$).
In summary, our method offers flexible selection with a focus either on simplicity, efficiency, or effectiveness, providing DR with complementary knowledge to reconstruct nuanced user preferences.

%Note that $a_{pu_j}$ is computed  in the same manner as $a_{ru_i}$.

\vspace{0.1cm}
\smallsection{Objective Function.}
Using the fine-grained representation of user preferences ${\hat{\mathbf{r}}_u}'$ derived in Eq. (\ref{eq:fg_obj}), the final objective of \proposed is reformulated from Eq.~\eqref{eq:diffrec_loss} as follows:
\begin{equation}    
\begin{aligned}
    \mathcal{L}_t = &\,\mathbb{E}_{\boldsymbol{q}\left(\textbf{x}_t \mid \textbf{x}_0\right)}\left[C\left\|{\hat{\mathbf{r}}_u}'-\textbf{r}_u\right\|_2^2\right].
\end{aligned}
\end{equation}


==> Source/Section/Preliminary.tex <==
\subsection{Diffusion Model}
The diffusion model is a probabilistic generative framework that reduces Gaussian noise iteratively. First, given an input data sample $x_0 \sim q(x_0)$, diffusion model gradually addes noise via forward process using a Gaussian distribution: 
\begin{align}
    q\left(x_t \mid x_{t-1}\right)=\mathcal{N}\left(x_t ; \sqrt{1-\beta_t} x_{t-1}, \beta_t I\right)
\end{align}
where $\beta_t$ represents the hyperparameter indicating the level of Gaussian noise at each timestep $t$. Using the reparameterization trick and the additivity between independent Gaussian distributions, we can directly define the Gaussian distribution that transitions from the initial state $x_0$ to a sample $x_t$ at an arbitrary time step $t$ in a closed form.
\begin{align}
    q\left(x_t \mid x_0\right)=\mathcal{N}\left(x_t ; \sqrt{\bar{\alpha}_t} x_0,\left(1-\bar{\alpha}_t\right) I\right)
    \label{forward}
\end{align}
where $\alpha_t = 1-\beta_t$ and $\bar{\alpha}_t = \prod_{t'=1}^{T} \alpha_{t'}$. 




Second, after finishing the forward process, the diffusion model removes the noise in reverse process using parameterized learned Gaussian distribution:
\begin{align}
    p_\theta(x_{t-1}|x_t) =
\mathcal{N}(\boldsymbol{\mu}_\theta(\mathbf{x_t, t}), \Sigma_\theta(\mathbf{x_t, t}))
\end{align}
At this point, $p_\theta(x_{t-1}|x_t)$ approximates the tractable forward process posteriors:

\begin{align}
& q\left(x_{t-1} \mid x_t, x_0\right) \propto \mathcal{N}\left(x_{t-1} ; \tilde{\boldsymbol{\mu}}\left(x_t, x_0, t\right), \sigma^2(t) I\right), \text { where } \\ & \left\{\begin{array}{l}\tilde{\boldsymbol{\mu}}\left(\boldsymbol{x}_t, x_0, t\right)=\frac{\sqrt{\alpha_t}\left(1-\bar{\alpha}_{t-1}\right)}{1-\bar{\alpha}_t} x_t+\frac{\sqrt{\bar{\alpha}_{t-1}}\left(1-\alpha_t\right)}{1-\bar{\alpha}_t} x_0, \\ \sigma^2(t)=\frac{\left(1-\alpha_t\right)\left(1-\bar{\alpha}_{t-1}\right)}{1-\bar{\alpha}_t}\end{array}\right.
\end{align}
Note that $\Sigma_\theta(\mathbf{x_t, t})$ is set as $\sigma^2(t)I$  for stable learning. The ultimate goal of the diffusion model is to learn the probability distribution of data $p_\theta(x_0) := \int p_\theta(x_{0:T})dx_{1:T}$, where \( p_\theta(x_{0:T}) := p(x_T) \prod^T_{t=1}p_\theta(x_{t-1}|x_t) \) represents the reverse process, denoising through a Markov chain with learned Gaussian transitions \cite{ho2020denoising}. Following this goal, diffusion models are trained by maximizing the variational bound, also known as the Evidence Lower Bound (ELBO), of the likelihood of the input data sample \(x_0\):

\begin{align}
 \log p\left(x_0\right)& = \log \int p\left(x_{0: T}\right) \mathrm{d} \boldsymbol{x}_{1: T} \nonumber \\ 
& =\log \mathbb{E}_{q\left(x_{1: T} \mid x_0\right)}\left[\frac{p\left(x_{0: T}\right)}{q\left(x_{1: T} \mid x_0\right)}\right] \nonumber \\
& \geq \underbrace{\mathbb{E}_{\boldsymbol{q}\left(\boldsymbol{x}_1 \mid \boldsymbol{x}_0\right)}\left[\log \boldsymbol{p}_{\boldsymbol{\theta}}\left(\boldsymbol{x}_0 \mid \boldsymbol{x}_1\right)\right]}_{\text {(reconstruction term) }}-\underbrace{D_{\mathrm{KL}}\left(\boldsymbol{q}\left(\boldsymbol{x}_T \mid \boldsymbol{x}_0\right) \| p\left(\boldsymbol{x}_T\right)\right)}_{\text {(prior matching term) }} \nonumber\\
& -\sum_{t=2}^T \underbrace{\mathbb{E}_{q\left(x_t \mid x_0\right)}\left[D_{\mathrm{KL}}\left(q\left(x_{t-1} \mid x_t, x_0\right) \| p_\theta\left(x_{t-1} \mid x_t\right)\right)\right]}_{\text {(denoising matching term) }} 
&
\end{align}

To train the parameter $\theta$, we only need to consider the reconstruction term and the denoising matching term. Among them, the denoising matching term can ultimately be characterized as minimizing the difference between the means of two distributions, and it can be formulated as follows:

\begin{align}
     &\mathbb{E}_{q\left(x_t \mid x_0\right)}\left[D_{\mathrm{KL}}\left(q\left(x_{t-1} \mid x_t, x_0\right) \| p_\theta\left(x_{t-1} \mid x_t\right)\right)\right] \nonumber\\ 
     = &\mathbb{E}_{q\left(x_t \mid x_0\right)}\left[\frac{1}{2 \sigma^2(t)}\left[\left\|\mu_\theta\left(x_t, t\right)-\tilde{\mu}\left(x_t, x_0, t\right)\right\|_2^2\right]\right]
     \label{eq7}
\end{align}
With the right reparameterization trick, the simplified diffusion model's final loss function is formulated as in Eq.~\eqref{eq7}:


\begin{align}
    \mathcal{L}_{simple} = \mathbb{E}_{t, \mathbf{x}_0, \boldsymbol{\epsilon}}\left[\left\|\boldsymbol{\epsilon}-\boldsymbol{\epsilon}_\theta\left(\sqrt{\bar{\alpha}_t} \mathbf{x}_0+\sqrt{1-\bar{\alpha}_t} \boldsymbol{\epsilon}, t\right)\right\|^2\right]
\end{align}
Note that the model is trained by predicting randomly sampled noises used at time step $t$. The details regarding the reconstruction term are omitted due to space constraints. After training the diffusion model, for data sampling, the model iteratively removes noise starting from Gaussian noise $\mathbf{x}_T \sim \mathcal{N}(0, I) \text{ to }\mathbf{x}_0$:

\begin{align}
& \mathbf{x}_{t-1} = \frac{1}{\sqrt{\alpha_t}}\left(\mathbf{x}_t - \frac{1 - \alpha_t}{\sqrt{1 - \bar{\alpha}_t}} \boldsymbol{\epsilon}_\theta\left(\mathbf{x}_t, t\right)\right) + \sigma_t \mathbf{z}, \quad \text{where} \\
& t = T, \ldots, 1 \text{ and } \mathbf{z} \sim \mathcal{N}(\mathbf{0}, \mathbf{I}) \quad \text{if } t > 1, \quad \text{else } \mathbf{z} = \mathbf{0} \nonumber
& 
\end{align}

\subsection{Diffusion Recommender Model}

Recently, there have been several attempts to apply diffusion to recommender systems, including sequential recommendation \cite{liu2023diffusion, yang2023generate}. However, this paper exclusively focuses on collaborative filtering, similar to DiffRec \cite{wang2023diffusion}. Unlike the original diffusion model, which predicts Gaussian noise $\epsilon$, DiffRec aims to predict observed input data $x_0$. The denoising matching term $\mathcal{L}$ is as follows:


\begin{align}
    \mathcal{L} = &\,\mathbb{E}_{q\left(x_t \mid x_0\right)}\left[\frac{1}{2 \sigma^2(t)}\left[\left\|\mu_\theta\left(x_t, t\right)-\tilde{\mu}\left(x_t, x_0, t\right)\right\|_2^2\right]\right] \nonumber\\
    =&\,\mathbb{E}_{\boldsymbol{q}\left(\boldsymbol{x}_t \mid \boldsymbol{x}_0\right)}\left[\frac{1}{2}\left(\frac{\bar{\alpha}_{t-1}}{1-\bar{\alpha}_{t-1}}-\frac{\bar{\alpha}_t}{1-\bar{\alpha}_t}\right)\left\|\hat{\boldsymbol{x}}_\theta\left(\boldsymbol{x}_t, t\right)-\boldsymbol{x}_0\right\|_2^2\right]
    \label{diffrec_loss}
\end{align}

Note that $\hat{\boldsymbol{x}}_\theta\left(\boldsymbol{x}_t, t\right)$ predict observed user-item interactions $x_0$. For sampling, Eq.~\eqref{forward} is used with small steps $T' < T$ to make $x_{T'}$, and the reverse process is performed using $\hat{x}_{t-1} = \mu_\theta\left(\hat{x}_t, t\right)$ for $t = T, \ldots, 1$, where $\hat{x}_{T}=x_{T'}$.





$$
q\left(\mathbf{x}_{t-1} \mid \mathbf{x}_t, \mathbf{x}_0\right)=\mathcal{N}(\mathbf{x}_{t-1} ; \tilde{\boldsymbol{\mu}}\left(\mathbf{x}_t, \mathbf{x}_0, \mathbf{t}\right), \sigma^2(t) \mathbf{I})
$$
where $\quad \tilde{\boldsymbol{\mu}}\left(\mathbf{x}_t, \mathbf{x}_0,\mathbf{t}\right):=\frac{\sqrt{\bar{\alpha}_{t-1}} (1-\alpha_t}{1-\bar{\alpha}_t} \mathbf{x}_0+\frac{\sqrt{\alpha_t}\left(1-\bar{\alpha}_{t-1}\right)}{1-\bar{\alpha}_t} \mathbf{x}_t \quad$ and $\quad \sigma^2(t):=\frac{(1-\alpha_t)(1-\bar{\alpha}_{t-1})}{1-\bar{\alpha}_t}$

At this point, $p_\theta(x_{t-1}|x_t)$ approximate the tractable forward process posteriors, $q_(x_{t-1}|x_t,x_0)$ = N(x_(t-1);

The diffusion model is a probabilistic generative model that gradually removes Gaussian noise, learning the probability distribution, \( p_\theta(x_0) := \int p_\theta(x_{0:T}) \), given an input data sample \( x_0 \sim q(x_0) \). Note that p_\theta(x_{0:T}) \) := p(x_t) \pi^T_{t=1}p_\theta(x_(t-1)|x_t) is the reverse process (denoising) consistof markov chain with learned guassian transistions. 



Diffusion model is probabilisitc generative model by graduallly removing the gaussian noise, which learns the problabiity distribution, p_\theta(x_0) := \int p_\theta(x_{0:T}, Given an input data sample x_0 ∼ q(x_0)

briefly review diffusion model





==> Source/Section/Preliminary_onlydiff.tex <==
\smallsection{Notations.}
We focus on collaborative filtering with implicit feedback \cite{hu2008collaborative}. Let $\mathcal{R} \in \{0, 1\}^{|\mathcal{U}| \times |\mathcal{I}|}$ be a binary rating matrix, where $\mathcal{U}$ and $\mathcal{I}$ are sets of users and items, respectively. The $u$-th row of $\mathcal{R}$, denoted as $\mathbf{r}_u \in \{0, 1\}^{|\mathcal{I}|}$, is the interaction history of user $u$. 
Let $\mathcal{M} \in \mathbb{R}^{|\mathcal{F}| \times |\mathcal{I}|}$ be an item feature matrix, where $\mathcal{F}$ is the set of distinct features.
In this paper, we treat $\mathcal{F}$ as words extracted from item reviews.
Each element $m_{fi}$ is the count of word $f$ for item $i$.

\smallsection{Diffusion-based recommender systems (DR)~\cite{wang2023diffusion}.}
We outline the forward, backward processes, training, and inference of DR:
%\vspace{-0.2cm}
\begin{itemize}[leftmargin=*]
    \item \textbf{Forward process.}
    During the forward process, the interaction history of user $u$ (i.e., $\mathbf{r}_u$) is treated as the input $\mathbf{x}_0$ at timestep $t = 0$. To make the reconstruction more robust, Gaussian noise is progressively added to $\mathbf{x}_0$ over $T$ timesteps, resulting in $\mathbf{x}_t$:
    \vspace{-0.2cm}
    \begin{equation}
        \begin{aligned}
            q\left(\mathbf{x}_t \mid \mathbf{x}_0\right)=\mathcal{N}\left(\mathbf{x}_t ; \sqrt{\bar{\alpha}_t} \mathbf{x}_0,\left(1-\bar{\alpha}_t\right) \boldsymbol{I}\right),
            \label{forward}
        \end{aligned}
    \vspace{-0.2cm}
    \end{equation}
    where $\bar{\alpha}_t = \prod_{t'=1}^{T} \alpha_{t'}$, and $\alpha_{t'}$ is a hyperparameter that controls the level of Gaussian noise added at timestep $t'$.

    \item \textbf{Backward process.}
    The backward process reconstructs the input step-by-step using a parameterized Markov chain $\theta$ that approximates the tractable forward process posteriors $q\left(\mathbf{x}_{t-1} \mid \mathbf{x}_t, \mathbf{x}_0\right)$:
    \vspace{-0.1cm}
    \begin{equation}
        \begin{aligned}
            p_\theta(\mathbf{x}_{t-1}|\mathbf{x}_t) &= \mathcal{N} (\boldsymbol{\mu}_\theta(\mathbf{x}_t, t), 
            \sigma^2(t)\mathbf{I}), \text{ where}\\
            %\Sigma_\theta(\mathbf{x}_t, t)) \\
            \boldsymbol{\mu}_\theta\left(\mathbf{x}_t, t\right)&=\frac{\sqrt{\alpha_t}\left(1-\bar{\alpha}_{t-1}\right)}{1-\bar{\alpha}_t} \mathbf{x}_t+\frac{\sqrt{\bar{\alpha}_{t-1}}\left(1-\alpha_t\right)}{1-\bar{\alpha}_t} \hat{\mathbf{x}}_\theta\left(\mathbf{x}_t, t\right).
        \end{aligned}
    \end{equation}
    
    \item \textbf{Training.}
    Basically, diffusion models~\cite{ho2020denoising} is trained by maximizing the Evidence Lower Bound of the log-likelihood of $\mathbf{x}_0$:
    \small{
        \begin{align}
        %  \log p\left(\textbf{x}_0\right) & = \log \int p\left(\textbf{x}_{0: T}\right) \mathrm{d} \textbf{x}_{1: T}  \nonumber \\  
        % & = \log \mathbb{E}_{q\left(\textbf{x}_{1: T} \mid \textbf{x}_0\right)}\left[\frac{p\left(\textbf{x}_{0: T}\right)}{q\left(\textbf{x}_{1: T} \mid \textbf{x}_0\right)}\right]  \nonumber \\ 
        % & \geq  \mathbb{E}_{q\left (\textbf{x}_{1: T} \mid \textbf{x}_0\right)}\left[ \log \frac{p\left(\textbf{x}_{0: T}\right)}{q\left(\textbf{x}_{1: T} \mid \textbf{x}_0\right)}\right]  \nonumber \\
        \log p(\mathbf{x}_0) & \geq \underbrace{\mathbb{E}_{q\left(\mathbf{x}_1 \mid \mathbf{x}_0\right)}\left[\log p_{\theta}\left(\mathbf{x}_0 \mid \mathbf{x}_1\right)\right]}_{\text {Reconstruction term }}-\underbrace{D_{\mathrm{KL}}\left(q\left(\mathbf{x}_T \mid \mathbf{x}_0\right) \| p\left(\mathbf{x}_T\right)\right)}_{\text {Prior matching term}} \nonumber \\
        & -\sum_{t=2}^T \underbrace{\mathbb{E}_{q\left(\mathbf{x}_t \mid \mathbf{x}_0\right)}\left[D_{\mathrm{KL}}\left(q\left(\mathbf{x}_{t-1} \mid \mathbf{x}_t, \mathbf{x}_0\right) \| p_\theta\left(\mathbf{x}_{t-1} \mid \mathbf{x}_t\right)\right)\right].}_{\text {Denoising matching term}}
    \end{align}
    }
    \normalsize
    Meanwhile, DR is simply optimized using the following loss:
    \begin{equation}\label{eq:diffrec_loss}
    \begin{aligned}
        \mathcal{L}_t = &\,\mathbb{E}_{\boldsymbol{q}\left(\textbf{x}_t \mid \textbf{x}_0\right)}\left[C\left\|\hat{\textbf{x}}_\theta\left(\textbf{x}_t, t\right)-\textbf{x}_0\right\|_2^2\right],
    \end{aligned}\vspace{-0.1cm}
    \end{equation}

    where $C = \frac{1}{2}\left(\frac{\bar{\alpha}_{t-1}}{1-\bar{\alpha}_{t-1}}-\frac{\bar{\alpha}_t}{1-\bar{\alpha}_t}\right)$, and  $\hat{\textbf{x}}_\theta\left(\textbf{x}_t, t\right)$ is the only component in DR, implemented as a Multi-Layer Perceptron (MLP).
    
    \vspace{0.15cm}
    \item \textbf{Inference.} After training $\theta$, the corrupted input $\mathbf{x}_t$ is iteratively denoised $\mathbf{x}_t \rightarrow \mathbf{x}_{t-1} \rightarrow \cdots \rightarrow \mathbf{x}_0$ by leveraging $p_\theta(\mathbf{x}_{t-1}|\mathbf{x}_t)$.

\end{itemize}

==> Source/Section/ProblemFormulation.tex <==
We focus on collaborative filtering with implicit feedback \cite{hu2008collaborative}. Let $\mathcal{R} \in \{0, 1\}^{|\mathcal{U}| \times |\mathcal{I}|}$ be a binary rating matrix, where $\mathcal{U}$ and $\mathcal{I}$ denote a set of users and items, respectively. The $u$-th row of $\mathcal{R}$, denoted as $\mathbf{r}_u \in \{0, 1\}^{|\mathcal{I}|}$, represents the interaction history of user $u$. 
Let $\mathcal{M} \in [0, 1]^{|\mathcal{F}| \times |\mathcal{I}|}$ be a feature matrix for item-side information, where $\mathcal{F}$ denotes the set of item features.
We construct $\mathcal{M}$ using item review words by computing a normalized bag-of-words histogram vector for each item (i.e., $0 \leq m_{ij} \leq 1, \forall i, j$). 
For instance, if a word $f$ appears in four items with counts $[2,0,3,0]$, normalizing by the total sum yields $\mathbf{m}_f = [0.4, 0.0, 0.6, 0.0]$.





Our objective is to develop a novel diffusion recommender model that effectively harnesses user-item interactions and item-side information to bridge the gap between diffusion models and recommender systems. 
% Our proposed model leverages the preferences of real users and pseudo-users established from item content features through a global attention mechanism to create fine-grained preferences for each user.
Our approach effectively mitigates the loss of personalized information stemming from noise accumulation during the forward process and seamlessly integrates rich item-side information into the user-oriented recommendation process.


% too much detailed?
% Let $\mathcal{R} \in \{0, 1\}^{|\mathcal{U}| \times |\mathcal{I}|}$ be a binary rating matrix, where $\mathcal{U}$ and $\mathcal{I}$ denote a set of users and items, respectively \cite{hu2008collaborative}. The $u$-th row of $\mathcal{R}$, denoted as $\mathbf{r}_u \in \{0, 1\}^{|\mathcal{I}|}$, represents the interaction history of user $u$ with items in $\mathcal{I}$. Let $\mathcal{F} \in [0, 1]^{|\mathcal{K}| \times |\mathcal{I}|}$ be a feature matrix for item-side information, where $\mathcal{K}$ denotes the set of item features\footnote{For convenience, we normalize item features such that $0 \leq f_{ij} \leq 1, \forall i, j$.}. Here, we define $\mathbf{f}_{u'} \in [0, 1]^{|\mathcal{I}|}$ as the interaction history of pseudo-user $u' \in \mathcal{K}$, since users' interaction histories can be viewed as co-visits of the items, same as $\mathbf{r}_u$.

% Our objective is to develop a new diffusion recommender model that fully utilizes generative abilities learned from the backward cascaded rating reconstruction. We incorporate global attention mechanisms for both real users and pseudo-users established from item content features. This rich semantic context helps address the loss of personalized information in user interactions caused by the continuous accumulation of noise throughout the forward process.


% previous
% In this paper, we focus on remmendation with implicit feedback \cite{hu2008collaborative}. Consider a system with $U$ users and $I$ items. The user-item interactions are denoted as a binary rating matrix $\mathbf{R} \in \{0, 1\}^{U \times I}$, where 
% the $u$-th row $\mathbf{r}_u \in \{0, 1\}^{I}$ denotes the interaction of user $u$ with the $I$ items. In addition, we denote item-side information as a feature matrix $\mathbf{F} \in \{0, 1\}^{K_{F} \times I}$, where the $i$-th column, i.e., $\mathbf{f}_{:,i}$, denotes the content feature of the $i$-th item. For convenience, we normalize the item features such that $0 < f_{ij} < 1, \forall i, j$. Our objective is to develop a new diffusion model-based recommender system, fully utilizing the generative and denoising ability of the diffusive process while introducing global attention to real users and item features to address the drawback of forgetting personalized information and sparsity issues to further enhance the performance.


% Not necessary for the problem formulation part.

% and feature-item matrix $S \in [0, 1]^{\mathcal{|F|} \times \mathcal{|I|}}$, respectively.  

% collaborative and item-side information , we can make user-item


% We define the pseudo user $f$'s item interaction vector as $S_f = \{s_{f1}, ..., s_{f\mathcal{I}}\}$.

% Let \( D: \mathcal{U} \times \mathcal{I} \rightarrow \mathbb{R}^{\mathcal{|U|} \times \mathcal{|I|}} \) represent the diffusion recommender. The 
% user \( u \) interest probability distribution is denoted as \( X_u \in \mathbb{R}^{\mathcal{|I|}} \), which is predicted by \( D(R_u) \). 
% Let $U^{real}_{u} = \{u' | \text{ top-k}(sim(R_u, R_{u'}))\}$ and $U^{pseudo}_{u} = \{f' | \text{ top-k}(sim(R_u, S_{f'}))\}$ be real and pseudo users for $u$, respectively. We define the pseudo users and real users as those who have the top-k most similar interests with user $u$ (a total of 2k users). 

% interests within the item space (i.e., $\hat{X_u}$) tailored for personalized recommendations to user $u$. This involves aggregating preference information from both real users $U^{real}_{u}$ and pseudo users $U^{pseudo}_{u}$, then combining them with the individual preference of user $u$

==> Source/Section/RelatedWork.tex <==
\subsection{Generative Recommender System}

briefly review Multi-VAE-based, GAN-based and existing diffusion mdoel-based recommender system

\subsection{Generative Recommender With Item Side information}
There are several studies incorporating item-side information into generative recommenders \cite{li2017collaborative, carraro2022conditioned}. This approach aims to overcome limitations of traditional deterministic collaborative filtering (CF) methods, enabling the effective capture of users’ complex, diverse, and uncertain interests within noisy and sparse user-item interactions. Additionally, by leveraging the context obtained from item-side information, deep latent representations of users and items can be generated, outperforming models that rely solely on user-item interactions.

==> Source/Section/test.tex <==
\begin{equation}
\begin{aligned}
& = \underbrace{\mathbb{E}_{q\left({x}_1 \mid x_0\right)}\left[\log p_{\theta}\left(x_0 \mid x_1\right)\right]}_{\text {(reconstruction term) }}-\underbrace{D_{\mathrm{KL}}\left(q\left(x_T \mid x_0\right) \| p\left(x_T\right)\right)}_{\text {(prior matching term) }}\\
& -\sum_{t=2}^T \underbrace{\mathbb{E}_{q\left(x_t \mid x_0\right)}\left[D_{\mathrm{KL}}\left(q\left(x_{t-1} \mid x_t, x_0\right) \| p_\theta\left(x_{t-1} \mid x_t\right)\right)\right],}_{\text {(denoising matching term) }} 
& 
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
& = \underbrace{\mathbb{E}_{q\left(\mathbf{x}__1 \mid \mathbf{x}_0\right)}\left[\log p{\theta}\left(\mathbf{x}_0 \mid \mathbf{x}_1\right)\right]}{\text {reconstruction term}}-\underbrace{D{\mathrm{KL}}\left(q\left(\mathbf{x}_T \mid \mathbf{x}_0\right) | p\left(\mathbf{x}_T\right)\right)}{\text {prior matching term}}\
& -\sum{t=2}^T \underbrace{\mathbb{E}{q\left(\mathbf{x}_t \mid \mathbf{x}_0\right)}\left[D{\mathrm{KL}}\left(q\left(\mathbf{x}_{t-1} \mid \mathbf{x}_t, \mathbf{x}_0\right) | p\theta\left(\mathbf{x}_{t-1} \mid \mathbf{x}_t\right)\right)\right]}{\text {denoising matching term}},
&
\end{aligned}
\end{equation}

==> Source/Table/ablation_topk.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
\begin{table}[t]
\renewcommand{\arraystretch}{0.85} % Reduces row height
\caption{Impact of varying the number of top-$K$ neighbors (rows) and pseudo-users (columns) across three datasets.}
\vspace{-1.0em}
\resizebox{0.85\linewidth}{!}{%
\begin{tabular}{c|c|cccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}}              & \multirow{2}{*}{\textbf{\#Top-$K$}} & \multicolumn{4}{c}{\textbf{\#Pseudo-users $(|\mathcal{F}|)$}}                                      \\ \cline{3-6} 
                                      &                         & \textbf{1,000}  & \textbf{5,000} & \textbf{10,000} & \textbf{20,000} \\ \hline\hline
\multirow{3}{*}{\textbf{Yelp}}        & \textbf{10}             & 0.1092          & 0.1077         & 0.1091          & 0.1115          \\
                                      & \textbf{20}             & 0.1123          & 0.1120          & 0.1117          & 0.1131          \\
                                      & \textbf{50}             & \textbf{0.1145} & 0.1136         & 0.1132          & 0.1133          \\ \hline
\multirow{3}{*}{\textbf{AM-Game}} & \textbf{10}             & 0.2134          & 0.2128         & 0.2151          & 0.2196          \\
                                      & \textbf{20}             & \textbf{0.2255} & 0.2155         & 0.2147          & 0.2142          \\
                                      & \textbf{50}             & 0.2207          & 0.2169         & 0.2191          & 0.2181          \\ \hline
\multirow{3}{*}{\textbf{Citeulike-t}} & \textbf{10}             & 0.1595          & 0.1594         & 0.1591          & 0.1603          \\
                                      & \textbf{20}             & 0.1584          & 0.1605         & \textbf{0.1616} & 0.1607          \\
                                      & \textbf{50}             & 0.1585          & 0.1566         & 0.1596          & 0.1572          \\ \bottomrule
\end{tabular}
}
\vspace{-0.4cm}
\label{topk}
\end{table}

==> Source/Table/acc_effi.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[t]
\renewcommand{\arraystretch}{1.1} % Reduces row height
\setlength{\abovecaptionskip}{1pt}   % 캡션과 테이블 간 위쪽 간격 제거
\centering
\renewcommand{\tabcolsep}{0.5mm} % Adjusts column spacing
\caption{Acc-efficiency comparison: DiffRec vs. CDiff4Rec.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|c|ccccccc}
\toprule
\textbf{Dataset}                       & \textbf{Model}                             & \textbf{R@10}                  & \textbf{R@50}                  & \textbf{R@100}                 & \textbf{N@10}                  & \textbf{N@50}                  & \textbf{N@100}                 & \textbf{\begin{tabular}[c]{@{}c@{}}Wall\\time\end{tabular}}              \\ \hline\hline
                                       & \textbf{DiffRec}                           & 0.0643                         & 0.1882                         & 0.2818                         & 0.0437                         & 0.0779                         & 0.0982                         & 0:37:47                         \\
\multirow{-2}{*}{\textbf{Yelp}}        & \cellcolor[HTML]{EFEFEF}\textbf{CDiff4Rec} & \cellcolor[HTML]{EFEFEF}0.0722 & \cellcolor[HTML]{EFEFEF}0.2027 & \cellcolor[HTML]{EFEFEF}0.2966 & \cellcolor[HTML]{EFEFEF}0.0490 & \cellcolor[HTML]{EFEFEF}0.0853 & \cellcolor[HTML]{EFEFEF}0.1057 & \cellcolor[HTML]{EFEFEF}0:41:45 \\ \hline
                                       & \textbf{DiffRec}                           & 0.1365                         & 0.3542                         & 0.4689                         & 0.0771                         & 0.1279                         & 0.1478                         & 0:25:13                         \\
\multirow{-2}{*}{\textbf{AM-Game}}     & \cellcolor[HTML]{EFEFEF}\textbf{CDiff4Rec} & \cellcolor[HTML]{EFEFEF}0.1442 & \cellcolor[HTML]{EFEFEF}0.3577 & \cellcolor[HTML]{EFEFEF}0.4813 & \cellcolor[HTML]{EFEFEF}0.0806 & \cellcolor[HTML]{EFEFEF}0.1299 & \cellcolor[HTML]{EFEFEF}0.1514 & \cellcolor[HTML]{EFEFEF}0:25:54 \\ \hline
                                       & \textbf{DiffRec}                           & 0.1175                         & 0.2270                         & 0.2826                         & 0.0748                         & 0.1008                         & 0.1109                         & 3:00:25                         \\
\multirow{-2}{*}{\textbf{Citeulike-t}} & \cellcolor[HTML]{EFEFEF}\textbf{CDiff4Rec} & \cellcolor[HTML]{EFEFEF}0.1177 & \cellcolor[HTML]{EFEFEF}0.2282 & \cellcolor[HTML]{EFEFEF}0.2838 & \cellcolor[HTML]{EFEFEF}0.0760 & \cellcolor[HTML]{EFEFEF}0.1019 & \cellcolor[HTML]{EFEFEF}0.1120 & \cellcolor[HTML]{EFEFEF}2:55:51 \\ \bottomrule
\end{tabular}
}
\vspace{-0.2cm}
\label{tab:acc_eff}
\end{table}

==> Source/Table/big_main_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}


\begin{table}[h]
  %\centering
  \caption{Overall performance comparison between the baselines and CDiff4Rec on three public datasets. The best results are highlighted in bold, and the second-best results are underlined. Statistical significance is denoted by *, **, and ***, indicating \(p \leq 0.05\), \(p \leq 0.005\), and \(p \leq 0.0005\) for the paired t-test versus the best baseline, respectively.}
  \vspace{-1.0em}
  \begin{adjustbox}{width=0.8\textwidth}
  \begin{tabular}{c|cc|cc|cc}
\hline
                                                        & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Yelp}} & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Amazon-game}}                   & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Citeulike-t}}                       \\
\multirow{-2}{*}{\textbf{Method}} & \textbf{R@20}                 & \textbf{N@20}              & \textbf{R@20}                            & \textbf{N@20}                            & \textbf{R@20}                             & \textbf{N@20}                              \\ \hline\hline
\textbf{LightGCN}                                       & 0.1047                        & 0.0553                     & \cellcolor[HTML]{FFFFFF}0.1899           & \cellcolor[HTML]{FFFFFF}0.0854           & \cellcolor[HTML]{FFFFFF}{\ul 0.1574}      & \cellcolor[HTML]{FFFFFF}{\ul 0.0800}         \\
\textbf{MF}                                             & 0.0918                        & 0.0485                     & \cellcolor[HTML]{FFFFFF}0.1839           & \cellcolor[HTML]{FFFFFF}0.0844           & \cellcolor[HTML]{FFFFFF}0.1535            & \cellcolor[HTML]{FFFFFF}0.0792             \\
\textbf{Ease}                                           & {\ul 0.1099}                  & {\ul 0.0601}               & \cellcolor[HTML]{FFFFFF}0.2108           & \cellcolor[HTML]{FFFFFF}0.1012           & \cellcolor[HTML]{FFFFFF}0.1359            & \cellcolor[HTML]{FFFFFF}0.0675             \\

\textbf{MultiVAE}                                            & 0.1056                        & 0.0548                     & \cellcolor[HTML]{FFFFFF}0.2181           & \cellcolor[HTML]{FFFFFF}0.0995           & \cellcolor[HTML]{FFFFFF}0.1447            & \cellcolor[HTML]{FFFFFF}0.0770              \\
\textbf{ConVAE}                                         & 0.1082                        & 0.0564                     & \cellcolor[HTML]{FFFFFF}0.2192           & \cellcolor[HTML]{FFFFFF}0.0997           & \cellcolor[HTML]{FFFFFF}0.1477            & \cellcolor[HTML]{FFFFFF}0.0775             \\
\rowcolor[HTML]{FFFFFF} 
\textbf{DiffRec}                                        & 0.1045                        & 0.0563                     & {\ul 0.2193}                             & {\ul 0.1034}                             & 0.1491                                    & 0.0791                                     \\ \hline
\textbf{Ours (+Real user)}                               & 0.1090                         & 0.0590                      & \cellcolor[HTML]{FFFFFF}0.2204           & \cellcolor[HTML]{FFFFFF}0.1033           & \cellcolor[HTML]{FFFFFF}0.1539            & \cellcolor[HTML]{FFFFFF}0.0822             \\
\textbf{Ours (+Pseudo user)}                               & 0.1074                        & 0.0584                     & \cellcolor[HTML]{FFFFFF}0.2250            & \cellcolor[HTML]{FFFFFF}\textbf{0.1054*} & \cellcolor[HTML]{FFFFFF}0.1605            & \cellcolor[HTML]{FFFFFF}0.0864             \\
\textbf{Ours (+Real \& Pseudo user)}                       & \textbf{0.1145***}            & \textbf{0.0622*}           & \cellcolor[HTML]{FFFFFF}\textbf{0.2255*} & \cellcolor[HTML]{FFFFFF}0.1052           & \cellcolor[HTML]{FFFFFF}\textbf{0.1616**} & \cellcolor[HTML]{FFFFFF}\textbf{0.0885***} \\ \hline
\end{tabular}  
  \end{adjustbox}
  \label{table:comparison}
\end{table}


==> Source/Table/dataset.tex <==
% WE DON'T NEED CORE INFO INTHE TABLE

\begin{table}[t]
\renewcommand{\arraystretch}{0.9} % Reduces row height
\caption{Statistics of the three public datasets.}
\vspace{-1.0em}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{ccccc}
\toprule
\textbf{Dataset}                        & \textbf{\#Users} & \textbf{\#Items} & \textbf{\#Interactions} & \textbf{Sparsity (\%)} \\ \hline\hline
\textbf{Yelp }        & 26,695  & 20,220  & 942,328        & 99.83 \\
\textbf{AM-Game } & 2,343   & 1,700   & 39,263         & 99.01 \\
\textbf{Citeulike-t}  & 7,947   & 25,975  & 132,275        & 99.94 \\ \bottomrule
\end{tabular}
}
\vspace{-0.5cm}
\label{Dataset}
\end{table}



==> Source/Table/small_main_table.tex <==
\begin{table}[t!]
    \renewcommand{\arraystretch}{0.9} % Reduces row height

    % \caption{Overall performance comparison between the baselines and CDiff4Rec on three public datasets. The best results are highlighted in bold, and the second-best results are underlined. Statistical significance is denoted by *, **, and ***, indicating \(p \leq 0.05\), \(p \leq 0.005\), and \(p \leq 0.0005\) for the paired t-test versus the best baseline, respectively.}
    \caption{The overall performance comparison.  *, **, and *** denote \(p \leq 0.05\), \(p \leq 0.005\), and \(p \leq 0.0005\) for the paired t-test on \proposed with the best baseline, respectively.}
    \captionsetup[subtable]{position=top}
    \vspace{-1em}
    \resizebox{0.4\textwidth}{!}{ 
    \begin{subtable}[t]{0.45\textwidth} % 너비를 \textwidth의 45%로 설정
    \centering
        \begin{tabular}{ccc}
            \toprule
\textbf{Yelp}                        & \textbf{R@20 }                 & \textbf{N@20 }                 \\ \midrule\midrule
LightGCN                             & 0.1047                & 0.0553                \\
BPRMF                                   & 0.0918                & 0.0485                \\
Ease                                 & {\ul 0.1099} & {\ul 0.0601} \\
MultiVAE                             & 0.1056                & 0.0548                \\
ConVAE                               & 0.1082                & 0.0564                \\
\rowcolor[HTML]{FFFFFF} 
DiffRec                     & 0.1045       & 0.0563       \\ \hline
\textbf{Ours (+Real users)}           & 0.1090                 & 0.0590                 \\
\textbf{Ours (+Pseudo-users)}         & 0.1074                & 0.0584                \\
\textbf{Ours (+Real \& Pseudo users)} & \textbf{0.1145***}    & \textbf{0.0622*}      \\ \bottomrule
\end{tabular}
    \end{subtable}
    }
    
    \vspace{0.5em}
    \resizebox{0.415\textwidth}{!}{ 
    \begin{subtable}[t]{0.45\textwidth} % 너비를 \textwidth의 45%로 설정
        \centering
        \begin{tabular}{ccc}
\textbf{Amazon-Game}                 & \textbf{R@20}                                     & \textbf{N@20}                                     \\ \hline\hline
LightGCN                             & \cellcolor[HTML]{FFFFFF}0.1899           & \cellcolor[HTML]{FFFFFF}0.0854           \\
BPRMF                                   & \cellcolor[HTML]{FFFFFF}0.1839           & \cellcolor[HTML]{FFFFFF}0.0844           \\
Ease                                 & \cellcolor[HTML]{FFFFFF}0.2108  & \cellcolor[HTML]{FFFFFF}0.1012  \\
MultiVAE                             & \cellcolor[HTML]{FFFFFF}0.2181           & \cellcolor[HTML]{FFFFFF}0.0995           \\
ConVAE                               & \cellcolor[HTML]{FFFFFF}0.2192           & \cellcolor[HTML]{FFFFFF}0.0997           \\
\rowcolor[HTML]{FFFFFF} 
DiffRec                     & {\ul 0.2193}                    & {\ul 0.1034}                    \\ \hline
\textbf{Ours (+Real users)}           & \cellcolor[HTML]{FFFFFF}0.2204           & \cellcolor[HTML]{FFFFFF}0.1033           \\
\textbf{Ours (+Pseudo-users)}         & \cellcolor[HTML]{FFFFFF}0.2250   & \cellcolor[HTML]{FFFFFF}\textbf{0.1054*} \\
\textbf{Ours (+Real \& Pseudo users)} & \cellcolor[HTML]{FFFFFF}\textbf{0.2255*} & \cellcolor[HTML]{FFFFFF}0.1052  \\ \bottomrule
\end{tabular}
    \end{subtable}
    }

\vspace{0.5em}
\resizebox{0.395\textwidth}{!}{ 
    \begin{subtable}[t]{0.45\textwidth} % 너비를 \textwidth의 45%로 설정
        \centering
        \begin{tabular}{ccc}
\textbf{Citeulike-t}                 & \textbf{R@20}                                      & \textbf{N@20}                                       \\ \hline\hline
LightGCN                             & \cellcolor[HTML]{FFFFFF}0.1574   & \cellcolor[HTML]{FFFFFF}0.0800    \\
BPRMF                                   & \cellcolor[HTML]{FFFFFF}0.1535            & \cellcolor[HTML]{FFFFFF}0.0792             \\
Ease                                 & \cellcolor[HTML]{FFFFFF}{\ul 0.1591}   & \cellcolor[HTML]{FFFFFF}{\ul 0.0852}    \\
MultiVAE                             & \cellcolor[HTML]{FFFFFF}0.1447            & \cellcolor[HTML]{FFFFFF}0.0770             \\
ConVAE                               & \cellcolor[HTML]{FFFFFF}0.1477            & \cellcolor[HTML]{FFFFFF}0.0775             \\
\rowcolor[HTML]{FFFFFF} 
DiffRec                     & 0.1491                     & 0.0791                      \\ \hline
\textbf{Ours (+Real users)}           & \cellcolor[HTML]{FFFFFF}0.1539            & \cellcolor[HTML]{FFFFFF}0.0822             \\
\textbf{Ours (+Pseudo-users)}         & \cellcolor[HTML]{FFFFFF}0.1605   & \cellcolor[HTML]{FFFFFF}0.0864    \\
\textbf{Ours (+Real \& Pseudo users)} & \cellcolor[HTML]{FFFFFF}\textbf{0.1616**} & \cellcolor[HTML]{FFFFFF}\textbf{0.0885***} \\ \bottomrule
\end{tabular}
\end{subtable}
}
\vspace{-0.4cm}
\label{tab:main_table}
\end{table}

==> Table/big_main_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}


\begin{table}[h]
  %\centering
  \caption{Overall performance comparison between the baselines and CDiff4Rec on three public datasets. The best results are highlighted in bold, and the second-best results are underlined. Statistical significance is denoted by *, **, and ***, indicating \(p \leq 0.05\), \(p \leq 0.005\), and \(p \leq 0.0005\) for the paired t-test versus the best baseline, respectively.}
  \vspace{-1.0em}
  \begin{adjustbox}{width=0.8\textwidth}
  \begin{tabular}{c|cc|cc|cc}
\hline
                                                        & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Yelp}} & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Amazon-game}}                   & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Citeulike-t}}                       \\
\multirow{-2}{*}{\textbf{Method}} & \textbf{R@20}                 & \textbf{N@20}              & \textbf{R@20}                            & \textbf{N@20}                            & \textbf{R@20}                             & \textbf{N@20}                              \\ \hline\hline
\textbf{LightGCN}                                       & 0.1047                        & 0.0553                     & \cellcolor[HTML]{FFFFFF}0.1899           & \cellcolor[HTML]{FFFFFF}0.0854           & \cellcolor[HTML]{FFFFFF}{\ul 0.1574}      & \cellcolor[HTML]{FFFFFF}{\ul 0.0800}         \\
\textbf{MF}                                             & 0.0918                        & 0.0485                     & \cellcolor[HTML]{FFFFFF}0.1839           & \cellcolor[HTML]{FFFFFF}0.0844           & \cellcolor[HTML]{FFFFFF}0.1535            & \cellcolor[HTML]{FFFFFF}0.0792             \\
\textbf{Ease}                                           & {\ul 0.1099}                  & {\ul 0.0601}               & \cellcolor[HTML]{FFFFFF}0.2108           & \cellcolor[HTML]{FFFFFF}0.1012           & \cellcolor[HTML]{FFFFFF}0.1359            & \cellcolor[HTML]{FFFFFF}0.0675             \\

\textbf{MultiVAE}                                            & 0.1056                        & 0.0548                     & \cellcolor[HTML]{FFFFFF}0.2181           & \cellcolor[HTML]{FFFFFF}0.0995           & \cellcolor[HTML]{FFFFFF}0.1447            & \cellcolor[HTML]{FFFFFF}0.0770              \\
\textbf{ConVAE}                                         & 0.1082                        & 0.0564                     & \cellcolor[HTML]{FFFFFF}0.2192           & \cellcolor[HTML]{FFFFFF}0.0997           & \cellcolor[HTML]{FFFFFF}0.1477            & \cellcolor[HTML]{FFFFFF}0.0775             \\
\rowcolor[HTML]{FFFFFF} 
\textbf{DiffRec}                                        & 0.1045                        & 0.0563                     & {\ul 0.2193}                             & {\ul 0.1034}                             & 0.1491                                    & 0.0791                                     \\ \hline
\textbf{Ours (+Real user)}                               & 0.1090                         & 0.0590                      & \cellcolor[HTML]{FFFFFF}0.2204           & \cellcolor[HTML]{FFFFFF}0.1033           & \cellcolor[HTML]{FFFFFF}0.1539            & \cellcolor[HTML]{FFFFFF}0.0822             \\
\textbf{Ours (+Pseudo user)}                               & 0.1074                        & 0.0584                     & \cellcolor[HTML]{FFFFFF}0.2250            & \cellcolor[HTML]{FFFFFF}\textbf{0.1054*} & \cellcolor[HTML]{FFFFFF}0.1605            & \cellcolor[HTML]{FFFFFF}0.0864             \\
\textbf{Ours (+Real \& Pseudo user)}                       & \textbf{0.1145***}            & \textbf{0.0622*}           & \cellcolor[HTML]{FFFFFF}\textbf{0.2255*} & \cellcolor[HTML]{FFFFFF}0.1052           & \cellcolor[HTML]{FFFFFF}\textbf{0.1616**} & \cellcolor[HTML]{FFFFFF}\textbf{0.0885***} \\ \hline
\end{tabular}  
  \end{adjustbox}
  \label{table:comparison}
\end{table}

